On variational iterative methods for semilinear problems

This paper presents an iterative method suitable for inverting semilinear problems which are important kernels in many numerical applications. The primary idea is to employ a parametrization that is able to reduce semilinear problems into linear systems which are solvable using fast Poisson solvers. Theoretical justifications are provided and supported by several experiments. Numerical results show that the method is not only computationally less expensive, but also yields accurate approximations.

==> LaTeX source files/manuscriptold.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE On the comparison of the Adomian decomposition and Picard Iteration
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}

There has been a long held controversy about the equivalence of the Adomian Decomposition Method and Picard Iteration. Even though  studies suggest that convergence of the Adomian Decomposition Method is faster than Picard Iteration and the quality of approximations is superior, recent investigations suggest otherwise. This work examines the performance of the two methods with semilinear boundary value problems which are important kernels in many numerical applications. Theoretical justifications are provided and supported by several numerical experiments. The test problems presented demonstrate that even though the two methods are distinctive, they produce approximations of nearly the same quality. However, the exponential convergence of the Adomian Decomposition Method suggested by some studies is not supported.
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the comparison between the Adomian decomposition (ADM) and Picard Iteration (PI) using the benchmark problem
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) = f,~~~~~&x\in \Omega,\\
\psi = \psi_D,~~~~~&x\in \Gamma_D,\\
-n\cdot \nabla \psi = g_N,~~~~~&x\in \Gamma_N.
\end{split}
\end{equation}
Here, $\Omega$ is a bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundary conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. 
%
\par In a variety of context, \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. They include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in some coordinate systems, which allow solutions to be written in closed form. However, the fundamental models governing most natural phenomena involving motion, diffusion, reaction, etc. occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of a numerical scheme with some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for the model problem \eqref{eq:bvp} do not always produce satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 
%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated. In many studies, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumptions on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito explored the existence of entire solutions by enforcing separability of $r$ and the unknown. He assumed that $r$ is expressible as $r = a(x)g(w)$, where $a$ is locally H\"older on $\R^n$ and $f$ (which is positive and nondecreasing for $w>0$) is a locally Lipschitz and continuous function on $\R^+$. In the said article, he established approximate range of the limit values of positive solutions. In later studies, his results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was also studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Infinitely many solutions may also exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory on nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible when major components of the mathematical model are trivialized, realistic models are relatively complicated and rarely admit closed form solutions. In spite of this, advances in differential and integro-differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods relies on the conjecture that solutions to nonlinear equations can be expressed as series. This leads to a set of explicit recursive relations governing the modes of the series. Methods of this sort are robust for approximating solutions to IVPs, but have been reformulated to adapt to boundary and initial boundary-value problems. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solutions. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par The Adomian Decomposition Method (ADM) has dominated the discussion about analytical methods recently. A lot of problems have been explored with the ADM and results were impressive. Interestingly, it is argued that in some tests the ADM yields the exact solution within few steps. This is debatable since those studies use simple functional forms of $r$.  This simplification makes it possible to write the series solution in closed form. What has not been discussed adequately is the fact that for complicated problems, the mode of the series may not be solvable analytically. Even if closed form expressions exist for the modes, it may not be possible to write the limit of the partial sum in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat misleading. One of the objectives of this study is to provide theoretical results on the convergence of the ADM from a variational perspective. This study also attempts to compare the ADM with Picard Iteration which shares a lot of conceptual and practical similarities. The remainder of the paper is organized as follows: Section \ref{sec:vf} discusses the weak and Galerkin approximation of \eqref{eq:bvp}. An iterative method is developed in Section \ref{eq:im} and compared with Picard Iteration. Theoretical results are also provided and supported by several test problems in Section \ref{sec:experiments}. Section \ref{sec:discusion} concludes the study with a brief overview of the performance of the ADM and Picard iteration.
%
\section{Weak formulation}\label{sec:wf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $\psi_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads:
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla u \cdot \nabla w \,\d x + \int_\Omega r(\cdot, u)w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x,~~ w \in H^1_\text{D}(\Omega).
\end{split}
\end{equation}
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,\psi) = r(\psi)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\subsection{Galerkin approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is:
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&\int_\Omega \nabla u_h \cdot \nabla w_h \,\d x + \int_\Omega r(\cdot, u_h)w_h \,\d x = \int_\Omega fw_h \d x + \int_{\Gamma_N} gw_h\, \d l - \int_\Omega \nabla \psi_{D,h} \cdot \nabla w_h\, \d x,~~w_h \in \mathcal{V}_{\text{D},h}^k.
\end{split}
\end{equation}
%
Here, $\psi_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is the nodal approximation of $\psi_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N,~|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
\psi_{D,h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. $\mathcal{A}$ is a square matrix and $\mathcal{B}(\bfs{\alpha})$, a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x~~~\text{and}~~~\mathcal{B}_\zeta(\bfs{\alpha}) = \int_\Omega r(\sum \alpha_z \phi_z) \phi_\zeta \,\d x.
\end{equation}
%
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ are also given by 
%
\begin{equation}
\beta_\zeta = \int_\Omega f\phi_{\zeta}\, dx,~~~~\gamma_\zeta = \int_{\Gamma_N} g \phi_{\zeta}\, dl,~~~~\mathcal{D}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x,~~~z \in Z,~\zeta \in \tilde{Z}.
\end{equation}
%
The Galerkin solution that approximates $\psi$ is written as
%
\begin{equation}
U = u_h + \psi_{D,h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix makes Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}\label{eq:im}
We furnish the weak form in \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem into a sequential inversion of the Laplacian. To begin, suppose that $\psi$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode $\psi_0$. Explicitly,
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} \mathcal{P}_\zeta
\end{equation}
%
where $\psi_\zeta,~\zeta \geq 0$ are to be determined. The terms $\mathcal{P}_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
\mathcal{P}_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $\mathcal{P}_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
 \sum_{\zeta \geq 0} \left(\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x + \int_\Omega \mathcal{P}_\zeta w \,\d x \right) = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x.
\end{equation}
%
The iterative scheme is developed by constructing the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ via matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem:
%
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&~\text{Find $\psi_\zeta = \varphi - \delta_{\zeta0}\psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x +  (1 - \delta_{\zeta0})\int_\Omega \mathcal{P}_\zeta w \,\d x = \delta_{\zeta0}\left(\int_\Omega fw \,\d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x\right)
\end{split}
\end{equation}
%
where $\varphi$ solve \eqref{eq:bvp} with $r = 0$, $\mathcal{P}_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, $\psi_0$ absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $\mathcal{P}_\zeta$ depends on $\psi_j,~ 0\leq j \leq \zeta-1$ only, $\mathcal{P}_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \sum_{\zeta \leq M} \psi_\zeta.
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved is summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  + \boldsymbol{F}_{\zeta-1} = 0$,~~where $\boldsymbol{F}_{\zeta z} = \int_\Omega \mathcal{P}_{\zeta} \phi_z \, \d x$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
Certainly, the ADM is attractive in the following ways: First, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. From \eqref{eq:adompolyn}, one observes that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grow exponentially. Also, a lot of memory is required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\subsection{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves the approximation of nonlinear equations by a sequence of explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the ADM and PI, where the majority of comparisons concluded that the ADM is the better of the two methods. Existing literature also suggest that the ADM is superconvergent (since it yields exact solutions within few iterations) and involves less computational work. This mischaracterization motivates some discussions in this study. First, analytical solutions are possible only when one is able to identify the partial solution with a familiar Taylor series. If the terms are mixed up and do not follow a recognizable series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:vf} generates the sequence $\{\tilde\psi_\zeta\}$ governed by the variational problem: 
%
\begin{equation}\label{eq:vfpicard}
\begin{split}
&~\text{Find $\tilde\psi_M = \varphi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \tilde\psi_M \cdot \nabla w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x - \int_\Omega r(\tilde\psi_{M-1})w \,\d x,
\end{split}
\end{equation}
%
for a specified beginning condition $\tilde\psi_{-1}$. The resulting Galerkin discrete problem is summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple test demonstrates that superiority of the ADM (as documented in some literature) is not supported and cannot be generalized.
%
\subsection{Example}\label{example:ex1} 
Consider the problem
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated exactly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x \mathcal{P}_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1,
\end{equation}
%
where $\mathcal{P}_\zeta$, associated with $r = \psi^2$, are given by 
%
\begin{equation*}
\mathcal{P}_0 = \psi_0^2,~~~~~\mathcal{P}_1 = 2\psi_0\psi_1,~~~~~\mathcal{P}_2 = \psi_1^2 + 2\psi_0\psi_2,~~\cdots.
\end{equation*}
After few evaluations, we obtain the the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which is recognized as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the exact solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha}. 
$$
It follows that 
$$
\lim_{M\to \infty} \frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1,\\
|x|,~&~\alpha = 1.\\
\end{cases}
$$
Thus, convergence is linear for the ADM. 
\par For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
If the beginning condition $\tilde\psi_{-1} = 0$ is supplied so that $\tilde\psi_0$ is consistent with ADM's zeroth mode, then $\tilde\psi_M$ is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the quality of PI approximations is better than ADM's. Overall, the convergence rate of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is subtle. The following results provide theoretical justifications that, for sufficient regularity conditions, the modes of the ADM are controlled and the partial solution converges to the exact solution.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $\psi_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, then 
$$
\| \nabla {\psi}_0\|_{L^{2}(\Omega)} \leq  C_{\Omega,0}\|f\|_{L^{2}(\Omega)} 
$$
and 
$$
\| \nabla {\psi}_\zeta\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta =1,2,\cdots,M
$$
%
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $\psi_\zeta$. It follows that  
%
\begin{equation*}
\| \nabla \hat{\psi}_M\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + \sum_{\zeta \leq M} C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation*}
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\hat{\psi}_M \to \psi$ in $H^1$ norm as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Now, since $\psi$ satisfy \eqref{eq:vf} and $\hat\psi_M$ satisfies
%
\begin{equation*}
\int_{\Omega} \nabla \hat\psi_M \cdot \nabla w\, \d x + \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x 
\end{equation*}
the error $e_M = \psi - \hat{\psi}_M$ satisfies
$$
\int_{\Omega} \nabla e_M \cdot \nabla w\, \d x = \int_\Omega r(\psi)w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \sum_{\zeta \geq M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x.
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, it holds that 
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)}. 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)}. 
$$
The theorem follows as $\sum_{\zeta \geq M} \mathcal{P}_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that whenever the zeroth mode of the ADM and the beginning condition of PI coincide, the two methods are identical as long as $r$ is linear. This result was first established by Golberg \cite{golberg1999note}. The major setback to his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}\label{lemm:lemmaadpisame}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $\mathcal{P}_\zeta = r(\psi_\zeta) = \psi_\zeta$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. After cancelling out common terms, we have 
%
\begin{equation*}
\begin{split}
\int_{\Omega} \nabla(\hat{\psi}_M - \tilde{\psi}_M) \cdot \nabla w\, \d x & = \int_{\Omega} \nabla \hat{\psi}_M\cdot \nabla w\, \d x - \int_{\Omega} \nabla \tilde{\psi}_M\cdot \nabla w\, \d x,\\
&=  \int_\Omega r(\tilde\psi_{M-1})w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x,\\
& =  \int_\Omega \tilde\psi_{M-1} w\,\d x - \int_\Omega \hat\psi_{M-1} w\,\d x.
\end{split}
\end{equation*}
%
The last equation is zero by assumption. As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to impose additional restrictions on $\mathcal{P}_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $\psi_D = 0$, it is known that there is at least one nontrivial solution. A quick exercise shows that $\mathcal{P}_\zeta = 0$ for all $\zeta$, and hence, the partial solution converges to the trivial solution. A trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely.
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the ADM and PI algorithms using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: Boundary conditions: $\psi_D = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; ~Nonlinearity: $r = -\sin \psi$; ~$f$: chosen appropriately;~Solution: $\psi = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6]$.\\[1ex]

\noindent
\textbf{Test 2}: Boundary conditions: $\psi = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~\psi = 0~\text{on}~\Gamma_{N}^R$ and $\psi = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$;~ Nonlinearity:  $r = -\psi$;~ $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$;~ Solution:~ $\psi = \cos(2\pi x) \sin(2\pi y)$.\\[1ex]

\noindent
\textbf{Test 3}: Boundary conditions: $\psi = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; Nonlinearity: $r = \psi - \psi^3$; ~$f$: chosen appropriately;~Solution $\psi = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Boundary conditions: $\psi = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $\psi = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$;~Nonlinearity: $r = -2\exp(\psi)$;~$f$: chosen appropriately;~Solution: $\psi = -2\ln[\cosh(0.25(2x-1)\theta)]/\cosh(0.25 \theta)$ where $\theta = 2\cosh(0.25 \theta)$.

\subsection{Numerical approximations}
For a fixed element area, the ADM and PI algorithms are run until the stopping criteria $\|\mathcal{R}(\hat\psi_M)\| \leq 10^{-10}$ and $\|\mathcal{R}(\tilde\psi_M)\| \leq 10^{-10}$ are met respectively.\\[1ex]
%


\newpage
\noindent
\textbf{Test 1}:\\
\vspace*{-0.15in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%

\newpage
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Number of iterations recorded for the ADM and PI for various number of elements.}}
\end{center}
%

\newpage
\subsection{Numerical convergence study}\label{sec:conv}
%
\vspace*{-0.3in}
We perform numerical convergence study of the ADM and PI.\\[1ex]
%
\noindent
\textbf{Test 1}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex1error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error1}
\end{centering}
\end{figure}
\vspace*{-0.1in}



%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex2error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error2}
\end{centering}
\end{figure}
\vspace*{-0.2in}

%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex3error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error3}
\end{centering}
\end{figure}
\vspace*{0.3in}


%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex4error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error4}
\end{centering}
\end{figure}

\subsection{Discussions and conclusion}\label{sec:discusion}
%
The numerical experiments show that the ADM approximations compare favorably with the analytical solutions. It is fascinating that the quality of the approximations obtained using the ADM and PI are commensurate. However, exponential convergence of the ADM suggested by some studies is not supported. For complicated nonlinearities however, the ADM is no more appealing as the associated polynomials are laborious to evaluate. In Test 3, the method fails to converge for $N = 8$ elements. The error $\|\mathcal{R}(\tilde\psi_M)\|_\infty$ plateaus out at $3.8462\times 10^{-3}$ and convergence is never attained, and additional terms scarcely improve the partial solution. It is noteworthy that this anomaly results from the numerical treatment but not a limitation of the method. 

\par The most important feature of the ADM revealed by this study is that convergence is generally linear and consistent with Picard iteration. In Test 2, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Lemma \ref{lemm:lemmaadpisame} and Golberg's conclusion holds. Indeed, the two schemes differ in scope but the quality of their approximations does not vary significantly. Contrary to the first three tests, Test 4 is intended to explore when PI can outperform the ADM. First of all, $\psi_0$ is the trivial solution. This leads to slow convergence of the associated Adomian polynomials. That is 
%
\begin{equation}\label{eq:bratuadompolyn}
\begin{split}
\mathcal{P}_0 & = 2\exp(\psi_0) = 2,\\
\mathcal{P}_1 & = 2 u_1 \exp(\psi_0) = 2 \psi_1,\\
\mathcal{P}_2 & = 2 u_2 \exp(\psi_0) + \psi_1^2 \exp(\psi_0) = 2 \psi_2 + \psi_1^2,\\ 
\mathcal{P}_3 & = \frac{1}{3}\psi_1^3 \exp(\psi_0) + 2\psi_3\exp(\psi_0) + 2\psi_1 \psi_2 \exp(\psi_0) = \frac{1}{3}\psi_1^3 + 2\psi_3 + 2\psi_1 \psi_2,
\end{split}
\end{equation}
and so on. Largely, the first mode of the partial solution inherits the most important features of the solution. As $\psi_0$ deviates significantly, convergence is affected adversely. One way to avoid this is to introduce, say, $f_1$ and $f_2$ into the differential equation such that $f_1 + f_2 = 0$. This way, the governing equation for $\psi_0$ may be written to have either $f_1$ as source term. $f_2$ is then expressed as a Taylor series and the terms are matched with the Adomian polynomials.\\[1ex]
%
\par The ADM and PI have been explored numerically from a variational context. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for exploring other nonlinear systems. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Even though the ADM is characterized as superconvergent, and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI.






\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}

==> LaTeX source files/update.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE A variational iterative scheme for semilinear boundary value problems
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}
This paper presents an iterative method for solving semilinear boundary-value problems, which are important kernels in many numerical applications. The method employs a decomposition that is able to reduce the original problem into a set of simpler problems which are easy to invert. For special boundary condition, the approach allows fast Poisson solvers to be engaged. Theoretical justifications are provided and supported by several numerical experiments. Results obtained suggest that the method is not only computationally attractive, but also produces accurate approximations.  
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the boundary-value problem (BVP)
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) &= f,~~~~~\,x\in \Omega,\\
\psi &= \psi_\alpha,~~~x\in \Gamma_D,\\
-n\cdot \nabla \psi &= g_N,~~~x\in \Gamma_N,
\end{split}
\end{equation}
where $\Omega$ is bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundaries conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. In a variety of context, the model in \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. These include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in most coordinate systems, which allows solutions to be written in closed form. However, the fundamental models governing most natural phenomena (involving combinations of motion, diffusion, reaction, etc) occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of some numerical scheme alongside some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for model problems of the form \eqref{eq:bvp} do not give satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 

%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated and chaotic. In many applications, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumption on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito investigated the existence of entire solutions by enforcing separability of $r$ in the spatial coordinates and the unknown. In particular, the form $r = a(x)g(w)$ was assumed, where $a$ is locally H\"older on $\R^n$ and $f$ is a locally Lipschitz continuous function on $\R^+$ which is positive and nondecreasing for $w>0$. In the said article, the author established approximate range of the limit values of positive solutions. Naito's results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Sometimes, infinitely many solutions exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory of nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible only when major components of the mathematical model are trivialized, realistic models are relatively complicated do not generally permit closed form solutions. In spite of this, advances in differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods is to conjecture that solutions to nonlinear equations can be expressed as infinite series. This leads to a set of explicit recursive relations governing the modes of the series. These methods are robust for approximating solutions to Cauchy problems but has been reformulated to adapt to boundary and initial boundary-value problems. In some test problems, these methods have been demonstrated to yield the exact solutions. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solution. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par It is debatable that the methods yield exact solutions in some problems because simple functional forms are used.  This simplification makes it possible to write the series solutions in closed forms. What has not been discussed adequately is the fact that for complicated problems, the systems governing each mode of the partial solution may not be solvable analytically. Moreover, even if closed form expressions exist for the modes, it may not be possible to write the limit of the approximation in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat subtle. One of the objectives of this study is to provide a variational framework for studying the convergence of the Adomian Decomposition Method (ADM) which shares a lot of similarities with other decomposition techniques. Once the framework is established, all finite element results follow readily. This study will also attempt to compare the ADM to Picard Iteration (PI). While the two methods are distinct in their conceptual and practical approaches, the later has been considered by some authors as superior. This study will compare the performance of the two methods numerically. The remainder of the paper is organized as follows: Section \ref{sec:motivation} provides a simple motivation which inspires this discussion. Section \ref{sec:vf} discusses the Galerkin approximation that is used to invert \eqref{eq:bvp}. The numerical procedures that use the Adomian decomposition and Picard Iteration are outlined in Section \ref{sec:discralg}. Section \ref{sec:experiments} explores several numerical experiments to compare the performance of the two methods; and Section \ref{sec:conclusion} concludes the study with a brief overview.
%















\section{Weak formulation}\label{sec:vf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $u_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - u_\text{D} \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&~a(u,w) + b(u; w)= \ell(w),~~~ \forall w \in H^1_\text{D}(\Omega),
\end{split}
\end{equation}
%
where
%
\begin{equation}\label{eq:vdef}
\begin{split}
&a(v,w) = (\nabla v, \nabla w),\\[1ex]
&b(v;w) = (r(\cdot,v), w),\\[1ex]
&\ell(w) = (f,w) - \langle g,w\rangle_N - a(u_D,w).
\end{split}
\end{equation}
%
Here, $(\cdot,\cdot)$ denotes the usual inner product in $L^2(\Omega)$ and $\langle \cdot, \cdot \rangle_N$ is
the inner product on $L^2(\Gamma_N)$. 
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,u) = r(u)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\section{Galerkin finite element approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&~a(u_h, w_h) + b(u_h; w_h) = \ell(w_h),~~~ \forall w_h \in \mathcal{V}_{\text{D},h}^k,
\end{split}
\end{equation}
%
where $a$ and $b$ satisfy \eqref{eq:vdef} and 
\begin{equation}
\ell(w_h) = (f,w_h) - \langle g, w_h \rangle_N - a(u_{D,h},w_h)
\end{equation}
%
Here, $u_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is used as an approximation (e.g. nodal interpolant) of $u_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N$ and $|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
u_{\text{D},h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. The matrix $\mathcal{A}$ is square and $\mathcal{B}(\bfs{\alpha})$ is a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} =  a(\phi_z, \phi_\zeta)~~~\text{and}~~~ \mathcal{B}_\zeta(\bfs{\alpha}) = b(\sum \alpha_z \phi_z; \phi_\zeta)
\end{equation}
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ also have entries 
%
\begin{equation}
\beta_\zeta = (f, \phi_{\zeta}),~~~~~\gamma_\zeta = \<g_N, \phi_{\zeta}\>_N,~~~~\mathcal{D}_{\zeta z} = a(\phi_z, \phi_\zeta),~~z \in Z,~\zeta \in \tilde{Z}
\end{equation}
%
The Galerkin finite element solution that approximates $\widetilde{u}$ is written as
%
\begin{equation}
\tilde{u}_h = u_h + u_{\text{D},h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix make Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}
We furnish the weak form \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem in \eqref{eq:vf} into a sequential inversion of the Laplacian. To begin, let $u$ satisfy \eqref{eq:bvp} and $v$ solve a similar problem with $r = 0$. Suppose in addition that $u$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode. That is
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} p_\zeta
\end{equation}
%
where $\psi_0$ (referred to as the zeroth) and $\psi_\zeta,~\zeta \geq 1$ are to be determined. The terms $p_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
p_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $p_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
a(\psi_0,w) + \sum _{\zeta \geq 1}\big[a(\psi_\zeta,w) + (p_{\zeta}, w)\big] = \ell(w).
\end{equation}
%
The iterative scheme is developed by finding the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ by matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&\text{Find $\psi_\zeta = v - \delta_{\zeta0}u_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&a(\psi_\zeta,w) + (1 - \delta_{\zeta0}) (p_{\zeta-1}, w) = \delta_{\zeta0}\ell(w),~~~\zeta = 0,1,2, \cdots.
\end{split}
\end{equation}
%
where $p_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, the zeroth mode absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $p_\zeta$ depends on $\psi_j,~ \leq j \leq \zeta-1$ only, $p_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \psi_0 + \sum_{\zeta \geq 1} \psi_\zeta
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved can be summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  = \bfs{\xi}_{\zeta-1}$,~~where ${\xi}_{\zeta z} = - (p_{\zeta}, \phi_z)$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \bfs{\Psi}_0 + \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
Certainly, the ADM is attractive in the following ways: First of all, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. However, it is observed that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grows exponentially. A lot of memory is also required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\section{Comparison with Picard Iteration}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. 
\par Another aspect of the ADM that has been mischaracterized is its convergence. The method has been portrayed as superconvergent by many authors even though this assessment is misleading for an arbitrary nonlinearity. In fact, a closed form solution is possible only when one is able to identify the function whose truncated Taylor series is represented by the partial solution. If the terms are mixed up and do not follow a recognizable Taylor series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:nonlinsys} generates the sequence $\{\tilde\psi_\zeta\}$ governed by 
%
\begin{equation}\label{eq:picarditer} 
\begin{split}
&\text{Find $\tilde\psi_M = v - \psi_D \in H^1_\text{D}(\Omega)$ satisfying }\\[1ex]
&a(\tilde\psi_\zeta,w) =  \ell(w) - (r(\tilde\psi_{\zeta-1}), w),~~~\forall w\in H^1_\text{D}(\Omega)
\end{split}
\end{equation}
%
for a specified beginning condition $u_0$. The resulting discrete problem can be summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple tests demonstrates that superiority of one of the methods is not definite generalizable.
%
\subsection{Example}\label{example:ex1} 
Consider the IVP
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated explicitly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta(x) = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x p_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1.
\end{equation}
%
where $p_\zeta$, associate with $r = \psi^2$, are given by 
%
\begin{equation*}
p_0 = \psi_0^2,~~~~~p_1 = 2\psi_0\psi_1,~~~~~p_2 = \psi_1^2 + 2\psi_0\psi_2
\end{equation*}
and so on. After a few evaluations, \eqref{eq:seriessol} leads to the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which one recognizes as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha} 
$$
Hence,
$$
\lim_{M\to \infty} \frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1\\
|x|,~&~\alpha = 1\\
\end{cases}
$$
Thus, convergence is linear. For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
The solution is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the the quality of PI approximations is better than ADM's. In essence, the rate of convergence of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is rather subtle. The following results provide some formal theoretical justifications of the method using the benchmark problem.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $p_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $U_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, it follows from  \eqref{eq:adommatchingun} that  
%
\begin{equation}\label{eq:stab}
\| \nabla \hat{\psi}_\zeta\|_{L^{2}(\Omega)} \leq  \delta_{\zeta0}C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + (1 - \delta_{\zeta0}) C_{\Omega,\zeta}\|p_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation}
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $U_\zeta$.
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\| \nabla (\psi - \hat{\psi}_M)\|_{L^2(\Omega)} \to 0$ as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Since $\psi$ solve \eqref{eq:vf} and $\hat{\psi}_M$ is a partial solution, it follows that 
%
$$
a(\hat\psi_M, w) + \sum_{\zeta < M} (p_\zeta, w) = \ell(w).
$$
Also, the truncation error $e_M = \psi - \hat{\psi}_M$ satisfies
%
$$
a(e_M,w) = b(\psi; w) - \sum_{\zeta < M} (p_\zeta, w) = \sum_{\zeta \geq M} (p_\zeta, w)
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, the following result holds:
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)} 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} 
$$
The theorem follows as $\sum_{\zeta \geq M} p_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that if the zeroth mode of the ADM and the beginning condition of PI coincide, then the two methods are identical as long as $r$ is linear. This results was first established by Golberg \cite{golberg1999note}. The major setback of his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $p_{\zeta} = r(\psi_{\zeta}) = \psi_{\zeta}$ for all $\zeta \geq 0$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. Then 
%
\begin{equation*}
\begin{split}
a(\hat{\psi}_M - \tilde{\psi}_M,w) &= a(\hat{\psi}_M,w) - a(\tilde{\psi}_M,w) \\
& = \Big(\ell(w) - \sum_{\zeta < M} (p_\zeta, w)\Big) -  \Big(\ell(w) - (r(\tilde{\psi}_{M-1}), w) \Big)\\
& = \Big(\ell(w) - \sum_{\zeta < M} (\psi_\zeta, w)\Big) -  \Big(\ell(w) -  (\tilde{\psi}_{M-1}, w) \Big)\\
& = (\tilde{\psi}_{M-1}, w) - (\hat{\psi}_{M-1}, w)\\
& = 0
\end{split}
\end{equation*}
%
As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to place restrictions on $p_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $u_D = 0$, it is known that there is at least one nontrivial solution. Here, $p_\zeta = 0$ for all $\zeta$, so the partial solution converges to the trivial solution. It is noteworthy that the trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely, for instance, by adding and and subtracting an artificial source term to unsure that the first mode is nonzero. 
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the algorithm above using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: This is a Sine-Gordon problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity is $r = -\sin u$ and $f$ is chosen such that the exact solution is 
$$
u = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6].
$$

\noindent
\textbf{Test 2}: A Helmholtz-type problem with boundary conditions $u = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~u = 0~\text{on}~\Gamma_{N}^R$ and $u = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$. Moreover, we set $r = u$ and $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$ so that the exact solution is 
$$
u = \cos(2\pi x) \sin(2\pi y).
$$

\noindent
\textbf{Test 3}: A Modified Ginzburg-Landau problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity $r = u - u^3$ is prescribed and $f$ is constructed accordingly such that the exact solution is $u = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Bratu problem with boundary conditions $ u = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $u = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$. We also set $r = -2\exp(u)$ and choose $f$ such that exact solution is 
$$
u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~\text{ where}~~\theta = 2\cosh(0.25 \theta)
$$

\subsection{Numerical approximations}
It is fascinating that numerical results produced by the ADM are almost identical to those obtained using Picard iteration. For this reason, an attempt is made to evaluate the performance (in terms of number of iterations and error) of the two methods. In particular, for a fixed element area, the ADM algorithm is run until the stopping criterion $\|\mathcal{R}(\sum_{m=0}^{M} U_m)\| \leq 10^{-10}$ is met. To match the the same operations with PI, we equate solving for one mode of the ADM approximation to one iteration of PI. The stopping criterion $\| \mathcal{R}(\boldsymbol  \alpha_{m})\|_\infty \leq 10^{-10}$ is used to for PI.\\[1ex]
%


\noindent
\textbf{Test 1}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
Except for $n = 8$ elements, the approximations from both methods are again consistent. Even though the ADM with $8$ elements has smaller error, the method fails to converge. In fact, $\|\mathcal{R}(\bfs{\alpha}_{m})\|_\infty$ plateaues out at $3.8462\times 10^{-3}$ and convergence is never attained. At this point, additional terms scarcely improve the partial solutions. This clearly results from the numerical treatment but not a limitation of the method.
%



\subsection{Numerical convergence study}\label{sec:conv}
%
We perform numerical convergence study of the ADM and PI.\\[1ex]
\noindent
\textbf{Test 1}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex1error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error1}
\end{figure}

%
\noindent
\textbf{Test 2}:\\
\subsubsection{Test 2:}
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex2error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error2}
\end{figure}

%
\noindent
\textbf{Test 3}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex3error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error3}
\end{figure}



%
\noindent
\textbf{Test 4}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex4error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error4}
\end{figure}
















\subsection{Discussions}\label{sec:discusion}

It is apparently that the exponential convergence of the Adomian decomposition suggested by some studies is not supported by these results. As iterated above, exponential convergence may be validated using simple one-dimensional Cauchy problems. For complicated nonlinearities however, the Adomian decomposition is no more appealing as the associated polynomials are are difficult to evaluate analytically. For BVPs, the exercises in this study confirms that convergence of the method is generally linear and almost consistent with Picard iteration, except when the first mode of the partial solution deviates significantly from the exact solution. Largely, the first mode inherits the most important features of the solution. As it departs from the exact solution substantially, not only do we observe a reduced convergence, accuracy is also affected adversely.  








%
Evidently, the approximations compare favorably with the exact solution. It is remarkable that the errors associated with the ADM and PI are commensurate  and consistently of the same order. However, the VADM (especially in 1D applications) sometimes show insignificant improvements over the PI. \\[1ex]



Unlike the former test, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Golberg's conclusion holds. The two schemes may differ in scope but their approximations do not vary significantly. \\[1ex] 
%



\section{Conclusion} \label{sec:conclusion}
The Adomian decomposition has been explored numerically from a variational context. While the method has been characterized as super convergent and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI. However, the test problems presented in this paper show that it is indeterminate to conclude that the ADM converges faster and provides superior approximations. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method completely avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems in lower and higher dimensions. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for other explorations. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Moreover, superior approximations and fast convergence of the ADM over its counterpart, the Picard Iteration, is not been supported by this study.\\[1ex] 






























































%We solve a modified stationary Ginzburg-Landau-type problem with homogeneous Dirichlet conditions. The nonlinear reaction is $r(x,u) = u - u^3$. As emphasized above, analytical solutions to this problem are unknown and non-unique. 
%Calculation of $\mathcal{P}_\zeta$ in this example is less tedious as it is easy to automatize the process. Simulation results are depicted in the following figure and table.

















\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}





%This procedure is summarized in the following table.
%%
%\begin{algorithm}[H]
%\caption{ADM procedure}
%\begin{algorithmic}
%\smallskip
%\State Find $u_0 = v - u_D \in H^1_\text{D}(\Omega)$ satisfying  $A(u_0,w) = L(w)$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\For{$\zeta = 1$} until convergence
%\smallskip
%\State Find $u_\zeta \in H^1_\text{D}(\Omega)$ satisfying  $A(u_\zeta,w) + J_{\zeta-1}(w) = 0$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\EndFor
%\smallskip
%\State Set $u = \sum_{\zeta=0}^\infty u_{\zeta}$.
%\end{algorithmic}\label{alg:adomianvf}
%\end{algorithm}














%\textbf{Example 1}
%Consider the Bratu problem 
%%
%\begin{equation}\label{eq:bratu}
%-u'' - 2\exp(u) = 0,~~u(0) = u(1) = 0.
%\end{equation}
%%
%with solution 
%\begin{equation*}
%u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~~~\text{where}~~~~\theta = 2\cosh(0.25 \theta)
%\end{equation*}
%%
%Clearly, the first mode of the ADM is trivial since it solves $-u_0'' = 0, ~u_0(0) = u_0(1) = 0$. Accordingly, the first few Adomian polynomials are 
%%
%\begin{equation}\label{eq:bratuadompolyn}
%\begin{split}
%p_0 & = 2\exp(u_0) = 2,\\
%p_1 & = 2 u_1 \exp(u_0) = 2 u_1,\\
%p_2 & = 2 u_2 \exp(u_0) + u_1^2 \exp(u_0) = 2 u_2 + u_1^2,\\ 
%\end{split}
%\end{equation}
%%
%and so on. One primary advantage of the ADM that comes handy is that we are able to calculate the modes exactly or semi-analytically. Here, the higher-order modes given explicitly by
%%
%\begin{equation}\label{eq:seriessol}
%u_\zeta = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
%\end{equation}
%%
%Table \ref{tab:adom1} shows the errors associated with the first five nontrivial partial solutions.
%%
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.88630(-02)& 7.38115(-03)& 3.13039(-03)& 1.39757(-03)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five partial solution.}}\label{tab:adom1}
%\end{center}
%%
%For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. Then,  the $M^{\text{th}}$-iterate is calculated according to
%%
%\begin{equation}\label{eq:pibratu}
%-\psi_M'' - 2\exp(\psi_{M-1}) = 0, ~~\text{with}~~~\psi_M(0) = \psi_M(1) = 0.
%\end{equation}
%%
%The solution follows \eqref{eq:seriessol} with $p_{\zeta-1}$ replaced by $\exp(\psi_{\zeta-1})$. However, except $\psi_0$, all higher-order iterates are available semi-analytically. The associated errors are also tabulate in Table \ref{tab:picard1}.
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\psi_M$  & $\psi_1$ & $\psi_2$ & $\psi_3$ & $\psi_4$ & $\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.45576(-02)& 3.89215(-03)& 1.04761(-03)& 2.82658(-04)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
%\end{center}
%%
%Apparently, the two schemes maintain the same order of accuracy. However, PI approximations show marginal gains over ADM's. This is because $u_0 \equiv 0$ leads to slow convergence of the associated polynomials (see \eqref{eq:bratuadompolyn}), which in turn results in loss in accuracy.



\section{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration (also known as simple or fixed-point iteration). Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. It has also been documented that the ADM converges exponentially. As mentioned earlier, majority of convergence studies used simple forms of $r$ which makes it possible to infer the exact solution from the first few partial solutions. This study does not attempt to unify the two methods. Rather, it provides the framework to appreciate the convergence rates of the two schemes. To provide a common ground and access the performance the schemes, we provide a simple tests to demonstrate that superiority of one of the methods is problem dependent and not generalizable.\\[1ex]
%
\textbf{Example 1}
Consider the modified stationary Gross-Pitaevskii problem
%
\begin{equation}
\begin{split}
-\psi'' - 2\psi^3 + \psi &= 0,~~x \in (0,1),\\[1ex]
\psi(0) = 1,~ \psi(1) &= 2e/(1+e^2)
\end{split}
\end{equation}
%
which is satisfied  by $\psi(x) = \sech x$. With $r = -2\psi^3 + \psi $, the associated Adomian polynomials are 
%
\begin{equation*}
\begin{split}
p_0 &= -2\psi_0^3 + \psi_0,\\
p_1 &= - 6\psi_1\psi_0^2 + \psi_1,\\
p_2 &= - 6\psi_2\psi_0^2 - 6\psi_0\psi_1^2 + \psi_2,
\end{split}
\end{equation*}
and so on. The zeroth mode solves 
$$
-\hat\psi_0'' = 0,~~~~\hat\psi_0(0) = 1,~ ~\hat\psi_0(1) = 2e/(1+e^2)
$$ 
with solution 
$$
\hat\psi_0(x) = (1 + (1 - x)e^2 - x + 2ex))/(1 + e^2)
$$
All higher order terms are calculated using
%
\begin{equation}\label{eq:gensol}
\hat\psi_\zeta(x) = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
\end{equation}
%
Table \ref{tab:adom1} shows the errors associated with the first five partial solutions.
%
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $6.51945(-03)$ & $2.86278(-03)$  & $1.33711(-03)$ \\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five partial solution calculated using $N = 64$ elements.}}\label{tab:adom1}
\end{center}
%
For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. The $M^{\text{th}}$-iterate satisfies
%
\begin{equation}\label{eq:pibratu}
-\tilde \psi_M'' - 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1} = 0, ~~\text{with}~~~\tilde \psi_M(0) = 1,~~\tilde \psi_M(1) = 2e/(1+e^2).
\end{equation}
%
The solution follows \eqref{eq:gensol} with $p_{\zeta-1}$ replaced by $- 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1}$. The associated errors are also tabulate in Table \ref{tab:picard1}.
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\tilde\psi_M$  & $\tilde\psi_1$ & $\tilde\psi_2$ & $\tilde\psi_3$ & $\tilde\psi_4$ & $\tilde\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $5.96274(-03)$ & $2.22830(-03)$ & $8.43414(-04)$\\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
\end{center}




==> Latex Source files/LaTeX source files/manuscriptold.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE On the comparison of the Adomian decomposition and Picard Iteration
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}

There has been a long held controversy about the equivalence of the Adomian Decomposition Method and Picard Iteration. Even though  studies suggest that convergence of the Adomian Decomposition Method is faster than Picard Iteration and the quality of approximations is superior, recent investigations suggest otherwise. This work examines the performance of the two methods with semilinear boundary value problems which are important kernels in many numerical applications. Theoretical justifications are provided and supported by several numerical experiments. The test problems presented demonstrate that even though the two methods are distinctive, they produce approximations of nearly the same quality. However, the exponential convergence of the Adomian Decomposition Method suggested by some studies is not supported.
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the comparison between the Adomian decomposition (ADM) and Picard Iteration (PI) using the benchmark problem
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) = f,~~~~~&x\in \Omega,\\
\psi = \psi_D,~~~~~&x\in \Gamma_D,\\
-n\cdot \nabla \psi = g_N,~~~~~&x\in \Gamma_N.
\end{split}
\end{equation}
Here, $\Omega$ is a bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundary conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. 
%
\par In a variety of context, \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. They include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in some coordinate systems, which allow solutions to be written in closed form. However, the fundamental models governing most natural phenomena involving motion, diffusion, reaction, etc. occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of a numerical scheme with some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for the model problem \eqref{eq:bvp} do not always produce satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 
%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated. In many studies, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumptions on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito explored the existence of entire solutions by enforcing separability of $r$ and the unknown. He assumed that $r$ is expressible as $r = a(x)g(w)$, where $a$ is locally H\"older on $\R^n$ and $f$ (which is positive and nondecreasing for $w>0$) is a locally Lipschitz and continuous function on $\R^+$. In the said article, he established approximate range of the limit values of positive solutions. In later studies, his results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was also studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Infinitely many solutions may also exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory on nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible when major components of the mathematical model are trivialized, realistic models are relatively complicated and rarely admit closed form solutions. In spite of this, advances in differential and integro-differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods relies on the conjecture that solutions to nonlinear equations can be expressed as series. This leads to a set of explicit recursive relations governing the modes of the series. Methods of this sort are robust for approximating solutions to IVPs, but have been reformulated to adapt to boundary and initial boundary-value problems. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solutions. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par The Adomian Decomposition Method (ADM) has dominated the discussion about analytical methods recently. A lot of problems have been explored with the ADM and results were impressive. Interestingly, it is argued that in some tests the ADM yields the exact solution within few steps. This is debatable since those studies use simple functional forms of $r$.  This simplification makes it possible to write the series solution in closed form. What has not been discussed adequately is the fact that for complicated problems, the mode of the series may not be solvable analytically. Even if closed form expressions exist for the modes, it may not be possible to write the limit of the partial sum in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat misleading. One of the objectives of this study is to provide theoretical results on the convergence of the ADM from a variational perspective. This study also attempts to compare the ADM with Picard Iteration which shares a lot of conceptual and practical similarities. The remainder of the paper is organized as follows: Section \ref{sec:vf} discusses the weak and Galerkin approximation of \eqref{eq:bvp}. An iterative method is developed in Section \ref{eq:im} and compared with Picard Iteration. Theoretical results are also provided and supported by several test problems in Section \ref{sec:experiments}. Section \ref{sec:discusion} concludes the study with a brief overview of the performance of the ADM and Picard iteration.
%
\section{Weak formulation}\label{sec:wf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $\psi_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads:
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla u \cdot \nabla w \,\d x + \int_\Omega r(\cdot, u)w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x,~~ w \in H^1_\text{D}(\Omega).
\end{split}
\end{equation}
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,\psi) = r(\psi)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\subsection{Galerkin approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is:
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&\int_\Omega \nabla u_h \cdot \nabla w_h \,\d x + \int_\Omega r(\cdot, u_h)w_h \,\d x = \int_\Omega fw_h \d x + \int_{\Gamma_N} gw_h\, \d l - \int_\Omega \nabla \psi_{D,h} \cdot \nabla w_h\, \d x,~~w_h \in \mathcal{V}_{\text{D},h}^k.
\end{split}
\end{equation}
%
Here, $\psi_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is the nodal approximation of $\psi_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N,~|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
\psi_{D,h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. $\mathcal{A}$ is a square matrix and $\mathcal{B}(\bfs{\alpha})$, a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x~~~\text{and}~~~\mathcal{B}_\zeta(\bfs{\alpha}) = \int_\Omega r(\sum \alpha_z \phi_z) \phi_\zeta \,\d x.
\end{equation}
%
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ are also given by 
%
\begin{equation}
\beta_\zeta = \int_\Omega f\phi_{\zeta}\, dx,~~~~\gamma_\zeta = \int_{\Gamma_N} g \phi_{\zeta}\, dl,~~~~\mathcal{D}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x,~~~z \in Z,~\zeta \in \tilde{Z}.
\end{equation}
%
The Galerkin solution that approximates $\psi$ is written as
%
\begin{equation}
U = u_h + \psi_{D,h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix makes Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}\label{eq:im}
We furnish the weak form in \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem into a sequential inversion of the Laplacian. To begin, suppose that $\psi$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode $\psi_0$. Explicitly,
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} \mathcal{P}_\zeta
\end{equation}
%
where $\psi_\zeta,~\zeta \geq 0$ are to be determined. The terms $\mathcal{P}_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
\mathcal{P}_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $\mathcal{P}_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
 \sum_{\zeta \geq 0} \left(\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x + \int_\Omega \mathcal{P}_\zeta w \,\d x \right) = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x.
\end{equation}
%
The iterative scheme is developed by constructing the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ via matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem:
%
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&~\text{Find $\psi_\zeta = \varphi - \delta_{\zeta0}\psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x +  (1 - \delta_{\zeta0})\int_\Omega \mathcal{P}_\zeta w \,\d x = \delta_{\zeta0}\left(\int_\Omega fw \,\d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x\right)
\end{split}
\end{equation}
%
where $\varphi$ solve \eqref{eq:bvp} with $r = 0$, $\mathcal{P}_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, $\psi_0$ absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $\mathcal{P}_\zeta$ depends on $\psi_j,~ 0\leq j \leq \zeta-1$ only, $\mathcal{P}_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \sum_{\zeta \leq M} \psi_\zeta.
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved is summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  + \boldsymbol{F}_{\zeta-1} = 0$,~~where $\boldsymbol{F}_{\zeta z} = \int_\Omega \mathcal{P}_{\zeta} \phi_z \, \d x$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
Certainly, the ADM is attractive in the following ways: First, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. From \eqref{eq:adompolyn}, one observes that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grow exponentially. Also, a lot of memory is required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\subsection{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves the approximation of nonlinear equations by a sequence of explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the ADM and PI, where the majority of comparisons concluded that the ADM is the better of the two methods. Existing literature also suggest that the ADM is superconvergent (since it yields exact solutions within few iterations) and involves less computational work. This mischaracterization motivates some discussions in this study. First, analytical solutions are possible only when one is able to identify the partial solution with a familiar Taylor series. If the terms are mixed up and do not follow a recognizable series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:vf} generates the sequence $\{\tilde\psi_\zeta\}$ governed by the variational problem: 
%
\begin{equation}\label{eq:vfpicard}
\begin{split}
&~\text{Find $\tilde\psi_M = \varphi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \tilde\psi_M \cdot \nabla w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x - \int_\Omega r(\tilde\psi_{M-1})w \,\d x,
\end{split}
\end{equation}
%
for a specified beginning condition $\tilde\psi_{-1}$. The resulting Galerkin discrete problem is summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple test demonstrates that superiority of the ADM (as documented in some literature) is not supported and cannot be generalized.
%
\subsection{Example}\label{example:ex1} 
Consider the problem
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated exactly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x \mathcal{P}_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1,
\end{equation}
%
where $\mathcal{P}_\zeta$, associated with $r = \psi^2$, are given by 
%
\begin{equation*}
\mathcal{P}_0 = \psi_0^2,~~~~~\mathcal{P}_1 = 2\psi_0\psi_1,~~~~~\mathcal{P}_2 = \psi_1^2 + 2\psi_0\psi_2,~~\cdots.
\end{equation*}
After few evaluations, we obtain the the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which is recognized as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the exact solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha}. 
$$
It follows that 
$$
\lim_{M\to \infty} \frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1,\\
|x|,~&~\alpha = 1.\\
\end{cases}
$$
Thus, convergence is linear for the ADM. 
\par For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
If the beginning condition $\tilde\psi_{-1} = 0$ is supplied so that $\tilde\psi_0$ is consistent with ADM's zeroth mode, then $\tilde\psi_M$ is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the quality of PI approximations is better than ADM's. Overall, the convergence rate of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is subtle. The following results provide theoretical justifications that, for sufficient regularity conditions, the modes of the ADM are controlled and the partial solution converges to the exact solution.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $\psi_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, then 
$$
\| \nabla {\psi}_0\|_{L^{2}(\Omega)} \leq  C_{\Omega,0}\|f\|_{L^{2}(\Omega)} 
$$
and 
$$
\| \nabla {\psi}_\zeta\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta =1,2,\cdots,M
$$
%
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $\psi_\zeta$. It follows that  
%
\begin{equation*}
\| \nabla \hat{\psi}_M\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + \sum_{\zeta \leq M} C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation*}
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\hat{\psi}_M \to \psi$ in $H^1$ norm as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Now, since $\psi$ satisfy \eqref{eq:vf} and $\hat\psi_M$ satisfies
%
\begin{equation*}
\int_{\Omega} \nabla \hat\psi_M \cdot \nabla w\, \d x + \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x 
\end{equation*}
the error $e_M = \psi - \hat{\psi}_M$ satisfies
$$
\int_{\Omega} \nabla e_M \cdot \nabla w\, \d x = \int_\Omega r(\psi)w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \sum_{\zeta \geq M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x.
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, it holds that 
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)}. 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)}. 
$$
The theorem follows as $\sum_{\zeta \geq M} \mathcal{P}_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that whenever the zeroth mode of the ADM and the beginning condition of PI coincide, the two methods are identical as long as $r$ is linear. This result was first established by Golberg \cite{golberg1999note}. The major setback to his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}\label{lemm:lemmaadpisame}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $\mathcal{P}_\zeta = r(\psi_\zeta) = \psi_\zeta$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. After cancelling out common terms, we have 
%
\begin{equation*}
\begin{split}
\int_{\Omega} \nabla(\hat{\psi}_M - \tilde{\psi}_M) \cdot \nabla w\, \d x & = \int_{\Omega} \nabla \hat{\psi}_M\cdot \nabla w\, \d x - \int_{\Omega} \nabla \tilde{\psi}_M\cdot \nabla w\, \d x,\\
&=  \int_\Omega r(\tilde\psi_{M-1})w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x,\\
& =  \int_\Omega \tilde\psi_{M-1} w\,\d x - \int_\Omega \hat\psi_{M-1} w\,\d x.
\end{split}
\end{equation*}
%
The last equation is zero by assumption. As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to impose additional restrictions on $\mathcal{P}_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $\psi_D = 0$, it is known that there is at least one nontrivial solution. A quick exercise shows that $\mathcal{P}_\zeta = 0$ for all $\zeta$, and hence, the partial solution converges to the trivial solution. A trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely.
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the ADM and PI algorithms using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: Boundary conditions: $\psi_D = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; ~Nonlinearity: $r = -\sin \psi$; ~$f$: chosen appropriately;~Solution: $\psi = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6]$.\\[1ex]

\noindent
\textbf{Test 2}: Boundary conditions: $\psi = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~\psi = 0~\text{on}~\Gamma_{N}^R$ and $\psi = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$;~ Nonlinearity:  $r = -\psi$;~ $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$;~ Solution:~ $\psi = \cos(2\pi x) \sin(2\pi y)$.\\[1ex]

\noindent
\textbf{Test 3}: Boundary conditions: $\psi = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; Nonlinearity: $r = \psi - \psi^3$; ~$f$: chosen appropriately;~Solution $\psi = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Boundary conditions: $\psi = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $\psi = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$;~Nonlinearity: $r = -2\exp(\psi)$;~$f$: chosen appropriately;~Solution: $\psi = -2\ln[\cosh(0.25(2x-1)\theta)]/\cosh(0.25 \theta)$ where $\theta = 2\cosh(0.25 \theta)$.

\subsection{Numerical approximations}
For a fixed element area, the ADM and PI algorithms are run until the stopping criteria $\|\mathcal{R}(\hat\psi_M)\| \leq 10^{-10}$ and $\|\mathcal{R}(\tilde\psi_M)\| \leq 10^{-10}$ are met respectively.\\[1ex]
%


\newpage
\noindent
\textbf{Test 1}:\\
\vspace*{-0.15in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%

\newpage
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Number of iterations recorded for the ADM and PI for various number of elements.}}
\end{center}
%

\newpage
\subsection{Numerical convergence study}\label{sec:conv}
%
\vspace*{-0.3in}
We perform numerical convergence study of the ADM and PI.\\[1ex]
%
\noindent
\textbf{Test 1}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex1error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error1}
\end{centering}
\end{figure}
\vspace*{-0.1in}



%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex2error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error2}
\end{centering}
\end{figure}
\vspace*{-0.2in}

%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex3error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error3}
\end{centering}
\end{figure}
\vspace*{0.3in}


%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex4error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error4}
\end{centering}
\end{figure}

\subsection{Discussions and conclusion}\label{sec:discusion}
%
The numerical experiments show that the ADM approximations compare favorably with the analytical solutions. It is fascinating that the quality of the approximations obtained using the ADM and PI are commensurate. However, exponential convergence of the ADM suggested by some studies is not supported. For complicated nonlinearities however, the ADM is no more appealing as the associated polynomials are laborious to evaluate. In Test 3, the method fails to converge for $N = 8$ elements. The error $\|\mathcal{R}(\tilde\psi_M)\|_\infty$ plateaus out at $3.8462\times 10^{-3}$ and convergence is never attained, and additional terms scarcely improve the partial solution. It is noteworthy that this anomaly results from the numerical treatment but not a limitation of the method. 

\par The most important feature of the ADM revealed by this study is that convergence is generally linear and consistent with Picard iteration. In Test 2, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Lemma \ref{lemm:lemmaadpisame} and Golberg's conclusion holds. Indeed, the two schemes differ in scope but the quality of their approximations does not vary significantly. Contrary to the first three tests, Test 4 is intended to explore when PI can outperform the ADM. First of all, $\psi_0$ is the trivial solution. This leads to slow convergence of the associated Adomian polynomials. That is 
%
\begin{equation}\label{eq:bratuadompolyn}
\begin{split}
\mathcal{P}_0 & = 2\exp(\psi_0) = 2,\\
\mathcal{P}_1 & = 2 u_1 \exp(\psi_0) = 2 \psi_1,\\
\mathcal{P}_2 & = 2 u_2 \exp(\psi_0) + \psi_1^2 \exp(\psi_0) = 2 \psi_2 + \psi_1^2,\\ 
\mathcal{P}_3 & = \frac{1}{3}\psi_1^3 \exp(\psi_0) + 2\psi_3\exp(\psi_0) + 2\psi_1 \psi_2 \exp(\psi_0) = \frac{1}{3}\psi_1^3 + 2\psi_3 + 2\psi_1 \psi_2,
\end{split}
\end{equation}
and so on. Largely, the first mode of the partial solution inherits the most important features of the solution. As $\psi_0$ deviates significantly, convergence is affected adversely. One way to avoid this is to introduce, say, $f_1$ and $f_2$ into the differential equation such that $f_1 + f_2 = 0$. This way, the governing equation for $\psi_0$ may be written to have either $f_1$ as source term. $f_2$ is then expressed as a Taylor series and the terms are matched with the Adomian polynomials.\\[1ex]
%
\par The ADM and PI have been explored numerically from a variational context. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for exploring other nonlinear systems. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Even though the ADM is characterized as superconvergent, and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI.






\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}

==> Latex Source files/LaTeX source files/update.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE A variational iterative scheme for semilinear boundary value problems
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}
This paper presents an iterative method for solving semilinear boundary-value problems, which are important kernels in many numerical applications. The method employs a decomposition that is able to reduce the original problem into a set of simpler problems which are easy to invert. For special boundary condition, the approach allows fast Poisson solvers to be engaged. Theoretical justifications are provided and supported by several numerical experiments. Results obtained suggest that the method is not only computationally attractive, but also produces accurate approximations.  
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the boundary-value problem (BVP)
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) &= f,~~~~~\,x\in \Omega,\\
\psi &= \psi_\alpha,~~~x\in \Gamma_D,\\
-n\cdot \nabla \psi &= g_N,~~~x\in \Gamma_N,
\end{split}
\end{equation}
where $\Omega$ is bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundaries conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. In a variety of context, the model in \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. These include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in most coordinate systems, which allows solutions to be written in closed form. However, the fundamental models governing most natural phenomena (involving combinations of motion, diffusion, reaction, etc) occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of some numerical scheme alongside some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for model problems of the form \eqref{eq:bvp} do not give satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 

%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated and chaotic. In many applications, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumption on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito investigated the existence of entire solutions by enforcing separability of $r$ in the spatial coordinates and the unknown. In particular, the form $r = a(x)g(w)$ was assumed, where $a$ is locally H\"older on $\R^n$ and $f$ is a locally Lipschitz continuous function on $\R^+$ which is positive and nondecreasing for $w>0$. In the said article, the author established approximate range of the limit values of positive solutions. Naito's results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Sometimes, infinitely many solutions exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory of nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible only when major components of the mathematical model are trivialized, realistic models are relatively complicated do not generally permit closed form solutions. In spite of this, advances in differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods is to conjecture that solutions to nonlinear equations can be expressed as infinite series. This leads to a set of explicit recursive relations governing the modes of the series. These methods are robust for approximating solutions to Cauchy problems but has been reformulated to adapt to boundary and initial boundary-value problems. In some test problems, these methods have been demonstrated to yield the exact solutions. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solution. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par It is debatable that the methods yield exact solutions in some problems because simple functional forms are used.  This simplification makes it possible to write the series solutions in closed forms. What has not been discussed adequately is the fact that for complicated problems, the systems governing each mode of the partial solution may not be solvable analytically. Moreover, even if closed form expressions exist for the modes, it may not be possible to write the limit of the approximation in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat subtle. One of the objectives of this study is to provide a variational framework for studying the convergence of the Adomian Decomposition Method (ADM) which shares a lot of similarities with other decomposition techniques. Once the framework is established, all finite element results follow readily. This study will also attempt to compare the ADM to Picard Iteration (PI). While the two methods are distinct in their conceptual and practical approaches, the later has been considered by some authors as superior. This study will compare the performance of the two methods numerically. The remainder of the paper is organized as follows: Section \ref{sec:motivation} provides a simple motivation which inspires this discussion. Section \ref{sec:vf} discusses the Galerkin approximation that is used to invert \eqref{eq:bvp}. The numerical procedures that use the Adomian decomposition and Picard Iteration are outlined in Section \ref{sec:discralg}. Section \ref{sec:experiments} explores several numerical experiments to compare the performance of the two methods; and Section \ref{sec:conclusion} concludes the study with a brief overview.
%















\section{Weak formulation}\label{sec:vf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $u_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - u_\text{D} \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&~a(u,w) + b(u; w)= \ell(w),~~~ \forall w \in H^1_\text{D}(\Omega),
\end{split}
\end{equation}
%
where
%
\begin{equation}\label{eq:vdef}
\begin{split}
&a(v,w) = (\nabla v, \nabla w),\\[1ex]
&b(v;w) = (r(\cdot,v), w),\\[1ex]
&\ell(w) = (f,w) - \langle g,w\rangle_N - a(u_D,w).
\end{split}
\end{equation}
%
Here, $(\cdot,\cdot)$ denotes the usual inner product in $L^2(\Omega)$ and $\langle \cdot, \cdot \rangle_N$ is
the inner product on $L^2(\Gamma_N)$. 
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,u) = r(u)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\section{Galerkin finite element approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&~a(u_h, w_h) + b(u_h; w_h) = \ell(w_h),~~~ \forall w_h \in \mathcal{V}_{\text{D},h}^k,
\end{split}
\end{equation}
%
where $a$ and $b$ satisfy \eqref{eq:vdef} and 
\begin{equation}
\ell(w_h) = (f,w_h) - \langle g, w_h \rangle_N - a(u_{D,h},w_h)
\end{equation}
%
Here, $u_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is used as an approximation (e.g. nodal interpolant) of $u_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N$ and $|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
u_{\text{D},h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. The matrix $\mathcal{A}$ is square and $\mathcal{B}(\bfs{\alpha})$ is a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} =  a(\phi_z, \phi_\zeta)~~~\text{and}~~~ \mathcal{B}_\zeta(\bfs{\alpha}) = b(\sum \alpha_z \phi_z; \phi_\zeta)
\end{equation}
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ also have entries 
%
\begin{equation}
\beta_\zeta = (f, \phi_{\zeta}),~~~~~\gamma_\zeta = \<g_N, \phi_{\zeta}\>_N,~~~~\mathcal{D}_{\zeta z} = a(\phi_z, \phi_\zeta),~~z \in Z,~\zeta \in \tilde{Z}
\end{equation}
%
The Galerkin finite element solution that approximates $\widetilde{u}$ is written as
%
\begin{equation}
\tilde{u}_h = u_h + u_{\text{D},h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix make Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}
We furnish the weak form \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem in \eqref{eq:vf} into a sequential inversion of the Laplacian. To begin, let $u$ satisfy \eqref{eq:bvp} and $v$ solve a similar problem with $r = 0$. Suppose in addition that $u$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode. That is
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} p_\zeta
\end{equation}
%
where $\psi_0$ (referred to as the zeroth) and $\psi_\zeta,~\zeta \geq 1$ are to be determined. The terms $p_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
p_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $p_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
a(\psi_0,w) + \sum _{\zeta \geq 1}\big[a(\psi_\zeta,w) + (p_{\zeta}, w)\big] = \ell(w).
\end{equation}
%
The iterative scheme is developed by finding the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ by matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&\text{Find $\psi_\zeta = v - \delta_{\zeta0}u_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&a(\psi_\zeta,w) + (1 - \delta_{\zeta0}) (p_{\zeta-1}, w) = \delta_{\zeta0}\ell(w),~~~\zeta = 0,1,2, \cdots.
\end{split}
\end{equation}
%
where $p_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, the zeroth mode absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $p_\zeta$ depends on $\psi_j,~ \leq j \leq \zeta-1$ only, $p_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \psi_0 + \sum_{\zeta \geq 1} \psi_\zeta
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved can be summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  = \bfs{\xi}_{\zeta-1}$,~~where ${\xi}_{\zeta z} = - (p_{\zeta}, \phi_z)$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \bfs{\Psi}_0 + \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
Certainly, the ADM is attractive in the following ways: First of all, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. However, it is observed that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grows exponentially. A lot of memory is also required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\section{Comparison with Picard Iteration}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. 
\par Another aspect of the ADM that has been mischaracterized is its convergence. The method has been portrayed as superconvergent by many authors even though this assessment is misleading for an arbitrary nonlinearity. In fact, a closed form solution is possible only when one is able to identify the function whose truncated Taylor series is represented by the partial solution. If the terms are mixed up and do not follow a recognizable Taylor series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:nonlinsys} generates the sequence $\{\tilde\psi_\zeta\}$ governed by 
%
\begin{equation}\label{eq:picarditer} 
\begin{split}
&\text{Find $\tilde\psi_M = v - \psi_D \in H^1_\text{D}(\Omega)$ satisfying }\\[1ex]
&a(\tilde\psi_\zeta,w) =  \ell(w) - (r(\tilde\psi_{\zeta-1}), w),~~~\forall w\in H^1_\text{D}(\Omega)
\end{split}
\end{equation}
%
for a specified beginning condition $u_0$. The resulting discrete problem can be summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple tests demonstrates that superiority of one of the methods is not definite generalizable.
%
\subsection{Example}\label{example:ex1} 
Consider the IVP
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated explicitly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta(x) = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x p_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1.
\end{equation}
%
where $p_\zeta$, associate with $r = \psi^2$, are given by 
%
\begin{equation*}
p_0 = \psi_0^2,~~~~~p_1 = 2\psi_0\psi_1,~~~~~p_2 = \psi_1^2 + 2\psi_0\psi_2
\end{equation*}
and so on. After a few evaluations, \eqref{eq:seriessol} leads to the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which one recognizes as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha} 
$$
Hence,
$$
\lim_{M\to \infty} \frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1\\
|x|,~&~\alpha = 1\\
\end{cases}
$$
Thus, convergence is linear. For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
The solution is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the the quality of PI approximations is better than ADM's. In essence, the rate of convergence of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is rather subtle. The following results provide some formal theoretical justifications of the method using the benchmark problem.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $p_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $U_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, it follows from  \eqref{eq:adommatchingun} that  
%
\begin{equation}\label{eq:stab}
\| \nabla \hat{\psi}_\zeta\|_{L^{2}(\Omega)} \leq  \delta_{\zeta0}C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + (1 - \delta_{\zeta0}) C_{\Omega,\zeta}\|p_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation}
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $U_\zeta$.
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\| \nabla (\psi - \hat{\psi}_M)\|_{L^2(\Omega)} \to 0$ as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Since $\psi$ solve \eqref{eq:vf} and $\hat{\psi}_M$ is a partial solution, it follows that 
%
$$
a(\hat\psi_M, w) + \sum_{\zeta < M} (p_\zeta, w) = \ell(w).
$$
Also, the truncation error $e_M = \psi - \hat{\psi}_M$ satisfies
%
$$
a(e_M,w) = b(\psi; w) - \sum_{\zeta < M} (p_\zeta, w) = \sum_{\zeta \geq M} (p_\zeta, w)
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, the following result holds:
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)} 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} 
$$
The theorem follows as $\sum_{\zeta \geq M} p_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that if the zeroth mode of the ADM and the beginning condition of PI coincide, then the two methods are identical as long as $r$ is linear. This results was first established by Golberg \cite{golberg1999note}. The major setback of his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $p_{\zeta} = r(\psi_{\zeta}) = \psi_{\zeta}$ for all $\zeta \geq 0$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. Then 
%
\begin{equation*}
\begin{split}
a(\hat{\psi}_M - \tilde{\psi}_M,w) &= a(\hat{\psi}_M,w) - a(\tilde{\psi}_M,w) \\
& = \Big(\ell(w) - \sum_{\zeta < M} (p_\zeta, w)\Big) -  \Big(\ell(w) - (r(\tilde{\psi}_{M-1}), w) \Big)\\
& = \Big(\ell(w) - \sum_{\zeta < M} (\psi_\zeta, w)\Big) -  \Big(\ell(w) -  (\tilde{\psi}_{M-1}, w) \Big)\\
& = (\tilde{\psi}_{M-1}, w) - (\hat{\psi}_{M-1}, w)\\
& = 0
\end{split}
\end{equation*}
%
As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to place restrictions on $p_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $u_D = 0$, it is known that there is at least one nontrivial solution. Here, $p_\zeta = 0$ for all $\zeta$, so the partial solution converges to the trivial solution. It is noteworthy that the trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely, for instance, by adding and and subtracting an artificial source term to unsure that the first mode is nonzero. 
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the algorithm above using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: This is a Sine-Gordon problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity is $r = -\sin u$ and $f$ is chosen such that the exact solution is 
$$
u = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6].
$$

\noindent
\textbf{Test 2}: A Helmholtz-type problem with boundary conditions $u = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~u = 0~\text{on}~\Gamma_{N}^R$ and $u = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$. Moreover, we set $r = u$ and $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$ so that the exact solution is 
$$
u = \cos(2\pi x) \sin(2\pi y).
$$

\noindent
\textbf{Test 3}: A Modified Ginzburg-Landau problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity $r = u - u^3$ is prescribed and $f$ is constructed accordingly such that the exact solution is $u = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Bratu problem with boundary conditions $ u = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $u = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$. We also set $r = -2\exp(u)$ and choose $f$ such that exact solution is 
$$
u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~\text{ where}~~\theta = 2\cosh(0.25 \theta)
$$

\subsection{Numerical approximations}
It is fascinating that numerical results produced by the ADM are almost identical to those obtained using Picard iteration. For this reason, an attempt is made to evaluate the performance (in terms of number of iterations and error) of the two methods. In particular, for a fixed element area, the ADM algorithm is run until the stopping criterion $\|\mathcal{R}(\sum_{m=0}^{M} U_m)\| \leq 10^{-10}$ is met. To match the the same operations with PI, we equate solving for one mode of the ADM approximation to one iteration of PI. The stopping criterion $\| \mathcal{R}(\boldsymbol  \alpha_{m})\|_\infty \leq 10^{-10}$ is used to for PI.\\[1ex]
%


\noindent
\textbf{Test 1}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
Except for $n = 8$ elements, the approximations from both methods are again consistent. Even though the ADM with $8$ elements has smaller error, the method fails to converge. In fact, $\|\mathcal{R}(\bfs{\alpha}_{m})\|_\infty$ plateaues out at $3.8462\times 10^{-3}$ and convergence is never attained. At this point, additional terms scarcely improve the partial solutions. This clearly results from the numerical treatment but not a limitation of the method.
%



\subsection{Numerical convergence study}\label{sec:conv}
%
We perform numerical convergence study of the ADM and PI.\\[1ex]
\noindent
\textbf{Test 1}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex1error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error1}
\end{figure}

%
\noindent
\textbf{Test 2}:\\
\subsubsection{Test 2:}
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex2error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error2}
\end{figure}

%
\noindent
\textbf{Test 3}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex3error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error3}
\end{figure}



%
\noindent
\textbf{Test 4}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex4error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error4}
\end{figure}
















\subsection{Discussions}\label{sec:discusion}

It is apparently that the exponential convergence of the Adomian decomposition suggested by some studies is not supported by these results. As iterated above, exponential convergence may be validated using simple one-dimensional Cauchy problems. For complicated nonlinearities however, the Adomian decomposition is no more appealing as the associated polynomials are are difficult to evaluate analytically. For BVPs, the exercises in this study confirms that convergence of the method is generally linear and almost consistent with Picard iteration, except when the first mode of the partial solution deviates significantly from the exact solution. Largely, the first mode inherits the most important features of the solution. As it departs from the exact solution substantially, not only do we observe a reduced convergence, accuracy is also affected adversely.  








%
Evidently, the approximations compare favorably with the exact solution. It is remarkable that the errors associated with the ADM and PI are commensurate  and consistently of the same order. However, the VADM (especially in 1D applications) sometimes show insignificant improvements over the PI. \\[1ex]



Unlike the former test, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Golberg's conclusion holds. The two schemes may differ in scope but their approximations do not vary significantly. \\[1ex] 
%



\section{Conclusion} \label{sec:conclusion}
The Adomian decomposition has been explored numerically from a variational context. While the method has been characterized as super convergent and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI. However, the test problems presented in this paper show that it is indeterminate to conclude that the ADM converges faster and provides superior approximations. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method completely avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems in lower and higher dimensions. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for other explorations. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Moreover, superior approximations and fast convergence of the ADM over its counterpart, the Picard Iteration, is not been supported by this study.\\[1ex] 






























































%We solve a modified stationary Ginzburg-Landau-type problem with homogeneous Dirichlet conditions. The nonlinear reaction is $r(x,u) = u - u^3$. As emphasized above, analytical solutions to this problem are unknown and non-unique. 
%Calculation of $\mathcal{P}_\zeta$ in this example is less tedious as it is easy to automatize the process. Simulation results are depicted in the following figure and table.

















\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}





%This procedure is summarized in the following table.
%%
%\begin{algorithm}[H]
%\caption{ADM procedure}
%\begin{algorithmic}
%\smallskip
%\State Find $u_0 = v - u_D \in H^1_\text{D}(\Omega)$ satisfying  $A(u_0,w) = L(w)$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\For{$\zeta = 1$} until convergence
%\smallskip
%\State Find $u_\zeta \in H^1_\text{D}(\Omega)$ satisfying  $A(u_\zeta,w) + J_{\zeta-1}(w) = 0$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\EndFor
%\smallskip
%\State Set $u = \sum_{\zeta=0}^\infty u_{\zeta}$.
%\end{algorithmic}\label{alg:adomianvf}
%\end{algorithm}














%\textbf{Example 1}
%Consider the Bratu problem 
%%
%\begin{equation}\label{eq:bratu}
%-u'' - 2\exp(u) = 0,~~u(0) = u(1) = 0.
%\end{equation}
%%
%with solution 
%\begin{equation*}
%u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~~~\text{where}~~~~\theta = 2\cosh(0.25 \theta)
%\end{equation*}
%%
%Clearly, the first mode of the ADM is trivial since it solves $-u_0'' = 0, ~u_0(0) = u_0(1) = 0$. Accordingly, the first few Adomian polynomials are 
%%
%\begin{equation}\label{eq:bratuadompolyn}
%\begin{split}
%p_0 & = 2\exp(u_0) = 2,\\
%p_1 & = 2 u_1 \exp(u_0) = 2 u_1,\\
%p_2 & = 2 u_2 \exp(u_0) + u_1^2 \exp(u_0) = 2 u_2 + u_1^2,\\ 
%\end{split}
%\end{equation}
%%
%and so on. One primary advantage of the ADM that comes handy is that we are able to calculate the modes exactly or semi-analytically. Here, the higher-order modes given explicitly by
%%
%\begin{equation}\label{eq:seriessol}
%u_\zeta = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
%\end{equation}
%%
%Table \ref{tab:adom1} shows the errors associated with the first five nontrivial partial solutions.
%%
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.88630(-02)& 7.38115(-03)& 3.13039(-03)& 1.39757(-03)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five partial solution.}}\label{tab:adom1}
%\end{center}
%%
%For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. Then,  the $M^{\text{th}}$-iterate is calculated according to
%%
%\begin{equation}\label{eq:pibratu}
%-\psi_M'' - 2\exp(\psi_{M-1}) = 0, ~~\text{with}~~~\psi_M(0) = \psi_M(1) = 0.
%\end{equation}
%%
%The solution follows \eqref{eq:seriessol} with $p_{\zeta-1}$ replaced by $\exp(\psi_{\zeta-1})$. However, except $\psi_0$, all higher-order iterates are available semi-analytically. The associated errors are also tabulate in Table \ref{tab:picard1}.
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\psi_M$  & $\psi_1$ & $\psi_2$ & $\psi_3$ & $\psi_4$ & $\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.45576(-02)& 3.89215(-03)& 1.04761(-03)& 2.82658(-04)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
%\end{center}
%%
%Apparently, the two schemes maintain the same order of accuracy. However, PI approximations show marginal gains over ADM's. This is because $u_0 \equiv 0$ leads to slow convergence of the associated polynomials (see \eqref{eq:bratuadompolyn}), which in turn results in loss in accuracy.



\section{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration (also known as simple or fixed-point iteration). Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. It has also been documented that the ADM converges exponentially. As mentioned earlier, majority of convergence studies used simple forms of $r$ which makes it possible to infer the exact solution from the first few partial solutions. This study does not attempt to unify the two methods. Rather, it provides the framework to appreciate the convergence rates of the two schemes. To provide a common ground and access the performance the schemes, we provide a simple tests to demonstrate that superiority of one of the methods is problem dependent and not generalizable.\\[1ex]
%
\textbf{Example 1}
Consider the modified stationary Gross-Pitaevskii problem
%
\begin{equation}
\begin{split}
-\psi'' - 2\psi^3 + \psi &= 0,~~x \in (0,1),\\[1ex]
\psi(0) = 1,~ \psi(1) &= 2e/(1+e^2)
\end{split}
\end{equation}
%
which is satisfied  by $\psi(x) = \sech x$. With $r = -2\psi^3 + \psi $, the associated Adomian polynomials are 
%
\begin{equation*}
\begin{split}
p_0 &= -2\psi_0^3 + \psi_0,\\
p_1 &= - 6\psi_1\psi_0^2 + \psi_1,\\
p_2 &= - 6\psi_2\psi_0^2 - 6\psi_0\psi_1^2 + \psi_2,
\end{split}
\end{equation*}
and so on. The zeroth mode solves 
$$
-\hat\psi_0'' = 0,~~~~\hat\psi_0(0) = 1,~ ~\hat\psi_0(1) = 2e/(1+e^2)
$$ 
with solution 
$$
\hat\psi_0(x) = (1 + (1 - x)e^2 - x + 2ex))/(1 + e^2)
$$
All higher order terms are calculated using
%
\begin{equation}\label{eq:gensol}
\hat\psi_\zeta(x) = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
\end{equation}
%
Table \ref{tab:adom1} shows the errors associated with the first five partial solutions.
%
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $6.51945(-03)$ & $2.86278(-03)$  & $1.33711(-03)$ \\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five partial solution calculated using $N = 64$ elements.}}\label{tab:adom1}
\end{center}
%
For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. The $M^{\text{th}}$-iterate satisfies
%
\begin{equation}\label{eq:pibratu}
-\tilde \psi_M'' - 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1} = 0, ~~\text{with}~~~\tilde \psi_M(0) = 1,~~\tilde \psi_M(1) = 2e/(1+e^2).
\end{equation}
%
The solution follows \eqref{eq:gensol} with $p_{\zeta-1}$ replaced by $- 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1}$. The associated errors are also tabulate in Table \ref{tab:picard1}.
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\tilde\psi_M$  & $\tilde\psi_1$ & $\tilde\psi_2$ & $\tilde\psi_3$ & $\tilde\psi_4$ & $\tilde\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $5.96274(-03)$ & $2.22830(-03)$ & $8.43414(-04)$\\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
\end{center}




==> Latex Source files/manuscriptold.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE On the comparison of the Adomian decomposition and Picard Iteration
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}

There has been a long held controversy about the equivalence of the Adomian Decomposition Method and Picard Iteration. Even though  studies suggest that convergence of the Adomian Decomposition Method is faster than Picard Iteration and the quality of approximations is superior, recent investigations suggest otherwise. This work examines the performance of the two methods with semilinear boundary value problems which are important kernels in many numerical applications. Theoretical justifications are provided and supported by several numerical experiments. The test problems presented demonstrate that even though the two methods are distinctive, they produce approximations of nearly the same quality. However, the exponential convergence of the Adomian Decomposition Method suggested by some studies is not supported.
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the comparison between the Adomian decomposition (ADM) and Picard Iteration (PI) using the benchmark problem
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) = f,~~~~~&x\in \Omega,\\
\psi = \psi_D,~~~~~&x\in \Gamma_D,\\
-n\cdot \nabla \psi = g_N,~~~~~&x\in \Gamma_N.
\end{split}
\end{equation}
Here, $\Omega$ is a bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundary conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. 
%
\par In a variety of context, \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. They include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in some coordinate systems, which allow solutions to be written in closed form. However, the fundamental models governing most natural phenomena involving motion, diffusion, reaction, etc. occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of a numerical scheme with some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for the model problem \eqref{eq:bvp} do not always produce satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 
%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated. In many studies, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumptions on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito explored the existence of entire solutions by enforcing separability of $r$ and the unknown. He assumed that $r$ is expressible as $r = a(x)g(w)$, where $a$ is locally H\"older on $\R^n$ and $f$ (which is positive and nondecreasing for $w>0$) is a locally Lipschitz and continuous function on $\R^+$. In the said article, he established approximate range of the limit values of positive solutions. In later studies, his results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was also studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Infinitely many solutions may also exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory on nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible when major components of the mathematical model are trivialized, realistic models are relatively complicated and rarely admit closed form solutions. In spite of this, advances in differential and integro-differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods relies on the conjecture that solutions to nonlinear equations can be expressed as series. This leads to a set of explicit recursive relations governing the modes of the series. Methods of this sort are robust for approximating solutions to IVPs, but have been reformulated to adapt to boundary and initial boundary-value problems. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solutions. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par The Adomian Decomposition Method (ADM) has dominated the discussion about analytical methods recently. A lot of problems have been explored with the ADM and results were impressive. Interestingly, it is argued that in some tests the ADM yields the exact solution within few steps. This is debatable since those studies use simple functional forms of $r$.  This simplification makes it possible to write the series solution in closed form. What has not been discussed adequately is the fact that for complicated problems, the mode of the series may not be solvable analytically. Even if closed form expressions exist for the modes, it may not be possible to write the limit of the partial sum in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat misleading. One of the objectives of this study is to provide theoretical results on the convergence of the ADM from a variational perspective. This study also attempts to compare the ADM with Picard Iteration which shares a lot of conceptual and practical similarities. The remainder of the paper is organized as follows: Section \ref{sec:vf} discusses the weak and Galerkin approximation of \eqref{eq:bvp}. An iterative method is developed in Section \ref{eq:im} and compared with Picard Iteration. Theoretical results are also provided and supported by several test problems in Section \ref{sec:experiments}. Section \ref{sec:discusion} concludes the study with a brief overview of the performance of the ADM and Picard iteration.
%
\section{Weak formulation}\label{sec:wf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $\psi_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads:
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla u \cdot \nabla w \,\d x + \int_\Omega r(\cdot, u)w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x,~~ w \in H^1_\text{D}(\Omega).
\end{split}
\end{equation}
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,\psi) = r(\psi)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\subsection{Galerkin approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is:
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&\int_\Omega \nabla u_h \cdot \nabla w_h \,\d x + \int_\Omega r(\cdot, u_h)w_h \,\d x = \int_\Omega fw_h \d x + \int_{\Gamma_N} gw_h\, \d l - \int_\Omega \nabla \psi_{D,h} \cdot \nabla w_h\, \d x,~~w_h \in \mathcal{V}_{\text{D},h}^k.
\end{split}
\end{equation}
%
Here, $\psi_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is the nodal approximation of $\psi_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N,~|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
\psi_{D,h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. $\mathcal{A}$ is a square matrix and $\mathcal{B}(\bfs{\alpha})$, a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x~~~\text{and}~~~\mathcal{B}_\zeta(\bfs{\alpha}) = \int_\Omega r(\sum \alpha_z \phi_z) \phi_\zeta \,\d x.
\end{equation}
%
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ are also given by 
%
\begin{equation}
\beta_\zeta = \int_\Omega f\phi_{\zeta}\, dx,~~~~\gamma_\zeta = \int_{\Gamma_N} g \phi_{\zeta}\, dl,~~~~\mathcal{D}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x,~~~z \in Z,~\zeta \in \tilde{Z}.
\end{equation}
%
The Galerkin solution that approximates $\psi$ is written as
%
\begin{equation}
U = u_h + \psi_{D,h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix makes Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}\label{eq:im}
We furnish the weak form in \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem into a sequential inversion of the Laplacian. To begin, suppose that $\psi$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode $\psi_0$. Explicitly,
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} \mathcal{P}_\zeta
\end{equation}
%
where $\psi_\zeta,~\zeta \geq 0$ are to be determined. The terms $\mathcal{P}_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
\mathcal{P}_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $\mathcal{P}_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
 \sum_{\zeta \geq 0} \left(\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x + \int_\Omega \mathcal{P}_\zeta w \,\d x \right) = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x.
\end{equation}
%
The iterative scheme is developed by constructing the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ via matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem:
%
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&~\text{Find $\psi_\zeta = \varphi - \delta_{\zeta0}\psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x +  (1 - \delta_{\zeta0})\int_\Omega \mathcal{P}_\zeta w \,\d x = \delta_{\zeta0}\left(\int_\Omega fw \,\d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x\right)
\end{split}
\end{equation}
%
where $\varphi$ solve \eqref{eq:bvp} with $r = 0$, $\mathcal{P}_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, $\psi_0$ absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $\mathcal{P}_\zeta$ depends on $\psi_j,~ 0\leq j \leq \zeta-1$ only, $\mathcal{P}_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \sum_{\zeta \leq M} \psi_\zeta.
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved is summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  + \boldsymbol{F}_{\zeta-1} = 0$,~~where $\boldsymbol{F}_{\zeta z} = \int_\Omega \mathcal{P}_{\zeta} \phi_z \, \d x$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
Certainly, the ADM is attractive in the following ways: First, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. From \eqref{eq:adompolyn}, one observes that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grow exponentially. Also, a lot of memory is required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\subsection{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves the approximation of nonlinear equations by a sequence of explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the ADM and PI, where the majority of comparisons concluded that the ADM is the better of the two methods. Existing literature also suggest that the ADM is superconvergent (since it yields exact solutions within few iterations) and involves less computational work. This mischaracterization motivates some discussions in this study. First, analytical solutions are possible only when one is able to identify the partial solution with a familiar Taylor series. If the terms are mixed up and do not follow a recognizable series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:vf} generates the sequence $\{\tilde\psi_\zeta\}$ governed by the variational problem: 
%
\begin{equation}\label{eq:vfpicard}
\begin{split}
&~\text{Find $\tilde\psi_M = \varphi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \tilde\psi_M \cdot \nabla w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x - \int_\Omega r(\tilde\psi_{M-1})w \,\d x,
\end{split}
\end{equation}
%
for a specified beginning condition $\tilde\psi_{-1}$. The resulting Galerkin discrete problem is summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple test demonstrates that superiority of the ADM (as documented in some literature) is not supported and cannot be generalized.
%
\subsection{Example}\label{example:ex1} 
Consider the problem
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated exactly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x \mathcal{P}_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1,
\end{equation}
%
where $\mathcal{P}_\zeta$, associated with $r = \psi^2$, are given by 
%
\begin{equation*}
\mathcal{P}_0 = \psi_0^2,~~~~~\mathcal{P}_1 = 2\psi_0\psi_1,~~~~~\mathcal{P}_2 = \psi_1^2 + 2\psi_0\psi_2,~~\cdots.
\end{equation*}
After few evaluations, we obtain the the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which is recognized as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the exact solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha}. 
$$
It follows that 
$$
\lim_{M\to \infty} \frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1,\\
|x|,~&~\alpha = 1.\\
\end{cases}
$$
Thus, convergence is linear for the ADM. 
\par For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
If the beginning condition $\tilde\psi_{-1} = 0$ is supplied so that $\tilde\psi_0$ is consistent with ADM's zeroth mode, then $\tilde\psi_M$ is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the quality of PI approximations is better than ADM's. Overall, the convergence rate of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is subtle. The following results provide theoretical justifications that, for sufficient regularity conditions, the modes of the ADM are controlled and the partial solution converges to the exact solution.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $\psi_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, then 
$$
\| \nabla {\psi}_0\|_{L^{2}(\Omega)} \leq  C_{\Omega,0}\|f\|_{L^{2}(\Omega)} 
$$
and 
$$
\| \nabla {\psi}_\zeta\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta =1,2,\cdots,M
$$
%
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $\psi_\zeta$. It follows that  
%
\begin{equation*}
\| \nabla \hat{\psi}_M\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + \sum_{\zeta \leq M} C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation*}
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\hat{\psi}_M \to \psi$ in $H^1$ norm as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Now, since $\psi$ satisfy \eqref{eq:vf} and $\hat\psi_M$ satisfies
%
\begin{equation*}
\int_{\Omega} \nabla \hat\psi_M \cdot \nabla w\, \d x + \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x 
\end{equation*}
the error $e_M = \psi - \hat{\psi}_M$ satisfies
$$
\int_{\Omega} \nabla e_M \cdot \nabla w\, \d x = \int_\Omega r(\psi)w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \sum_{\zeta \geq M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x.
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, it holds that 
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)}. 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)}. 
$$
The theorem follows as $\sum_{\zeta \geq M} \mathcal{P}_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that whenever the zeroth mode of the ADM and the beginning condition of PI coincide, the two methods are identical as long as $r$ is linear. This result was first established by Golberg \cite{golberg1999note}. The major setback to his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}\label{lemm:lemmaadpisame}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $\mathcal{P}_\zeta = r(\psi_\zeta) = \psi_\zeta$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. After cancelling out common terms, we have 
%
\begin{equation*}
\begin{split}
\int_{\Omega} \nabla(\hat{\psi}_M - \tilde{\psi}_M) \cdot \nabla w\, \d x & = \int_{\Omega} \nabla \hat{\psi}_M\cdot \nabla w\, \d x - \int_{\Omega} \nabla \tilde{\psi}_M\cdot \nabla w\, \d x,\\
&=  \int_\Omega r(\tilde\psi_{M-1})w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x,\\
& =  \int_\Omega \tilde\psi_{M-1} w\,\d x - \int_\Omega \hat\psi_{M-1} w\,\d x.
\end{split}
\end{equation*}
%
The last equation is zero by assumption. As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to impose additional restrictions on $\mathcal{P}_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $\psi_D = 0$, it is known that there is at least one nontrivial solution. A quick exercise shows that $\mathcal{P}_\zeta = 0$ for all $\zeta$, and hence, the partial solution converges to the trivial solution. A trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely.
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the ADM and PI algorithms using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: Boundary conditions: $\psi_D = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; ~Nonlinearity: $r = -\sin \psi$; ~$f$: chosen appropriately;~Solution: $\psi = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6]$.\\[1ex]

\noindent
\textbf{Test 2}: Boundary conditions: $\psi = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~\psi = 0~\text{on}~\Gamma_{N}^R$ and $\psi = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$;~ Nonlinearity:  $r = -\psi$;~ $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$;~ Solution:~ $\psi = \cos(2\pi x) \sin(2\pi y)$.\\[1ex]

\noindent
\textbf{Test 3}: Boundary conditions: $\psi = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; Nonlinearity: $r = \psi - \psi^3$; ~$f$: chosen appropriately;~Solution $\psi = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Boundary conditions: $\psi = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $\psi = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$;~Nonlinearity: $r = -2\exp(\psi)$;~$f$: chosen appropriately;~Solution: $\psi = -2\ln[\cosh(0.25(2x-1)\theta)]/\cosh(0.25 \theta)$ where $\theta = 2\cosh(0.25 \theta)$.

\subsection{Numerical approximations}
For a fixed element area, the ADM and PI algorithms are run until the stopping criteria $\|\mathcal{R}(\hat\psi_M)\| \leq 10^{-10}$ and $\|\mathcal{R}(\tilde\psi_M)\| \leq 10^{-10}$ are met respectively.\\[1ex]
%


\newpage
\noindent
\textbf{Test 1}:\\
\vspace*{-0.15in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%

\newpage
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Number of iterations recorded for the ADM and PI for various number of elements.}}
\end{center}
%

\newpage
\subsection{Numerical convergence study}\label{sec:conv}
%
\vspace*{-0.3in}
We perform numerical convergence study of the ADM and PI.\\[1ex]
%
\noindent
\textbf{Test 1}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex1error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error1}
\end{centering}
\end{figure}
\vspace*{-0.1in}



%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex2error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error2}
\end{centering}
\end{figure}
\vspace*{-0.2in}

%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex3error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error3}
\end{centering}
\end{figure}
\vspace*{0.3in}


%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex4error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error4}
\end{centering}
\end{figure}

\subsection{Discussions and conclusion}\label{sec:discusion}
%
The numerical experiments show that the ADM approximations compare favorably with the analytical solutions. It is fascinating that the quality of the approximations obtained using the ADM and PI are commensurate. However, exponential convergence of the ADM suggested by some studies is not supported. For complicated nonlinearities however, the ADM is no more appealing as the associated polynomials are laborious to evaluate. In Test 3, the method fails to converge for $N = 8$ elements. The error $\|\mathcal{R}(\tilde\psi_M)\|_\infty$ plateaus out at $3.8462\times 10^{-3}$ and convergence is never attained, and additional terms scarcely improve the partial solution. It is noteworthy that this anomaly results from the numerical treatment but not a limitation of the method. 

\par The most important feature of the ADM revealed by this study is that convergence is generally linear and consistent with Picard iteration. In Test 2, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Lemma \ref{lemm:lemmaadpisame} and Golberg's conclusion holds. Indeed, the two schemes differ in scope but the quality of their approximations does not vary significantly. Contrary to the first three tests, Test 4 is intended to explore when PI can outperform the ADM. First of all, $\psi_0$ is the trivial solution. This leads to slow convergence of the associated Adomian polynomials. That is 
%
\begin{equation}\label{eq:bratuadompolyn}
\begin{split}
\mathcal{P}_0 & = 2\exp(\psi_0) = 2,\\
\mathcal{P}_1 & = 2 u_1 \exp(\psi_0) = 2 \psi_1,\\
\mathcal{P}_2 & = 2 u_2 \exp(\psi_0) + \psi_1^2 \exp(\psi_0) = 2 \psi_2 + \psi_1^2,\\ 
\mathcal{P}_3 & = \frac{1}{3}\psi_1^3 \exp(\psi_0) + 2\psi_3\exp(\psi_0) + 2\psi_1 \psi_2 \exp(\psi_0) = \frac{1}{3}\psi_1^3 + 2\psi_3 + 2\psi_1 \psi_2,
\end{split}
\end{equation}
and so on. Largely, the first mode of the partial solution inherits the most important features of the solution. As $\psi_0$ deviates significantly, convergence is affected adversely. One way to avoid this is to introduce, say, $f_1$ and $f_2$ into the differential equation such that $f_1 + f_2 = 0$. This way, the governing equation for $\psi_0$ may be written to have either $f_1$ as source term. $f_2$ is then expressed as a Taylor series and the terms are matched with the Adomian polynomials.\\[1ex]
%
\par The ADM and PI have been explored numerically from a variational context. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for exploring other nonlinear systems. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Even though the ADM is characterized as superconvergent, and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI.






\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}

==> Latex Source files/update.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE A variational iterative scheme for semilinear boundary value problems
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}
This paper presents an iterative method for solving semilinear boundary-value problems, which are important kernels in many numerical applications. The method employs a decomposition that is able to reduce the original problem into a set of simpler problems which are easy to invert. For special boundary condition, the approach allows fast Poisson solvers to be engaged. Theoretical justifications are provided and supported by several numerical experiments. Results obtained suggest that the method is not only computationally attractive, but also produces accurate approximations.  
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the boundary-value problem (BVP)
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) &= f,~~~~~\,x\in \Omega,\\
\psi &= \psi_\alpha,~~~x\in \Gamma_D,\\
-n\cdot \nabla \psi &= g_N,~~~x\in \Gamma_N,
\end{split}
\end{equation}
where $\Omega$ is bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundaries conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. In a variety of context, the model in \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. These include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in most coordinate systems, which allows solutions to be written in closed form. However, the fundamental models governing most natural phenomena (involving combinations of motion, diffusion, reaction, etc) occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of some numerical scheme alongside some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for model problems of the form \eqref{eq:bvp} do not give satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 

%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated and chaotic. In many applications, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumption on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito investigated the existence of entire solutions by enforcing separability of $r$ in the spatial coordinates and the unknown. In particular, the form $r = a(x)g(w)$ was assumed, where $a$ is locally H\"older on $\R^n$ and $f$ is a locally Lipschitz continuous function on $\R^+$ which is positive and nondecreasing for $w>0$. In the said article, the author established approximate range of the limit values of positive solutions. Naito's results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Sometimes, infinitely many solutions exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory of nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible only when major components of the mathematical model are trivialized, realistic models are relatively complicated do not generally permit closed form solutions. In spite of this, advances in differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods is to conjecture that solutions to nonlinear equations can be expressed as infinite series. This leads to a set of explicit recursive relations governing the modes of the series. These methods are robust for approximating solutions to Cauchy problems but has been reformulated to adapt to boundary and initial boundary-value problems. In some test problems, these methods have been demonstrated to yield the exact solutions. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solution. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par It is debatable that the methods yield exact solutions in some problems because simple functional forms are used.  This simplification makes it possible to write the series solutions in closed forms. What has not been discussed adequately is the fact that for complicated problems, the systems governing each mode of the partial solution may not be solvable analytically. Moreover, even if closed form expressions exist for the modes, it may not be possible to write the limit of the approximation in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat subtle. One of the objectives of this study is to provide a variational framework for studying the convergence of the Adomian Decomposition Method (ADM) which shares a lot of similarities with other decomposition techniques. Once the framework is established, all finite element results follow readily. This study will also attempt to compare the ADM to Picard Iteration (PI). While the two methods are distinct in their conceptual and practical approaches, the later has been considered by some authors as superior. This study will compare the performance of the two methods numerically. The remainder of the paper is organized as follows: Section \ref{sec:motivation} provides a simple motivation which inspires this discussion. Section \ref{sec:vf} discusses the Galerkin approximation that is used to invert \eqref{eq:bvp}. The numerical procedures that use the Adomian decomposition and Picard Iteration are outlined in Section \ref{sec:discralg}. Section \ref{sec:experiments} explores several numerical experiments to compare the performance of the two methods; and Section \ref{sec:conclusion} concludes the study with a brief overview.
%















\section{Weak formulation}\label{sec:vf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $u_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - u_\text{D} \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&~a(u,w) + b(u; w)= \ell(w),~~~ \forall w \in H^1_\text{D}(\Omega),
\end{split}
\end{equation}
%
where
%
\begin{equation}\label{eq:vdef}
\begin{split}
&a(v,w) = (\nabla v, \nabla w),\\[1ex]
&b(v;w) = (r(\cdot,v), w),\\[1ex]
&\ell(w) = (f,w) - \langle g,w\rangle_N - a(u_D,w).
\end{split}
\end{equation}
%
Here, $(\cdot,\cdot)$ denotes the usual inner product in $L^2(\Omega)$ and $\langle \cdot, \cdot \rangle_N$ is
the inner product on $L^2(\Gamma_N)$. 
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,u) = r(u)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\section{Galerkin finite element approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&~a(u_h, w_h) + b(u_h; w_h) = \ell(w_h),~~~ \forall w_h \in \mathcal{V}_{\text{D},h}^k,
\end{split}
\end{equation}
%
where $a$ and $b$ satisfy \eqref{eq:vdef} and 
\begin{equation}
\ell(w_h) = (f,w_h) - \langle g, w_h \rangle_N - a(u_{D,h},w_h)
\end{equation}
%
Here, $u_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is used as an approximation (e.g. nodal interpolant) of $u_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N$ and $|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
u_{\text{D},h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. The matrix $\mathcal{A}$ is square and $\mathcal{B}(\bfs{\alpha})$ is a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} =  a(\phi_z, \phi_\zeta)~~~\text{and}~~~ \mathcal{B}_\zeta(\bfs{\alpha}) = b(\sum \alpha_z \phi_z; \phi_\zeta)
\end{equation}
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ also have entries 
%
\begin{equation}
\beta_\zeta = (f, \phi_{\zeta}),~~~~~\gamma_\zeta = \<g_N, \phi_{\zeta}\>_N,~~~~\mathcal{D}_{\zeta z} = a(\phi_z, \phi_\zeta),~~z \in Z,~\zeta \in \tilde{Z}
\end{equation}
%
The Galerkin finite element solution that approximates $\widetilde{u}$ is written as
%
\begin{equation}
\tilde{u}_h = u_h + u_{\text{D},h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix make Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}
We furnish the weak form \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem in \eqref{eq:vf} into a sequential inversion of the Laplacian. To begin, let $u$ satisfy \eqref{eq:bvp} and $v$ solve a similar problem with $r = 0$. Suppose in addition that $u$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode. That is
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} p_\zeta
\end{equation}
%
where $\psi_0$ (referred to as the zeroth) and $\psi_\zeta,~\zeta \geq 1$ are to be determined. The terms $p_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
p_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $p_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
a(\psi_0,w) + \sum _{\zeta \geq 1}\big[a(\psi_\zeta,w) + (p_{\zeta}, w)\big] = \ell(w).
\end{equation}
%
The iterative scheme is developed by finding the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ by matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&\text{Find $\psi_\zeta = v - \delta_{\zeta0}u_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&a(\psi_\zeta,w) + (1 - \delta_{\zeta0}) (p_{\zeta-1}, w) = \delta_{\zeta0}\ell(w),~~~\zeta = 0,1,2, \cdots.
\end{split}
\end{equation}
%
where $p_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, the zeroth mode absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $p_\zeta$ depends on $\psi_j,~ \leq j \leq \zeta-1$ only, $p_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \psi_0 + \sum_{\zeta \geq 1} \psi_\zeta
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved can be summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  = \bfs{\xi}_{\zeta-1}$,~~where ${\xi}_{\zeta z} = - (p_{\zeta}, \phi_z)$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \bfs{\Psi}_0 + \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
Certainly, the ADM is attractive in the following ways: First of all, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. However, it is observed that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grows exponentially. A lot of memory is also required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\section{Comparison with Picard Iteration}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. 
\par Another aspect of the ADM that has been mischaracterized is its convergence. The method has been portrayed as superconvergent by many authors even though this assessment is misleading for an arbitrary nonlinearity. In fact, a closed form solution is possible only when one is able to identify the function whose truncated Taylor series is represented by the partial solution. If the terms are mixed up and do not follow a recognizable Taylor series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:nonlinsys} generates the sequence $\{\tilde\psi_\zeta\}$ governed by 
%
\begin{equation}\label{eq:picarditer} 
\begin{split}
&\text{Find $\tilde\psi_M = v - \psi_D \in H^1_\text{D}(\Omega)$ satisfying }\\[1ex]
&a(\tilde\psi_\zeta,w) =  \ell(w) - (r(\tilde\psi_{\zeta-1}), w),~~~\forall w\in H^1_\text{D}(\Omega)
\end{split}
\end{equation}
%
for a specified beginning condition $u_0$. The resulting discrete problem can be summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple tests demonstrates that superiority of one of the methods is not definite generalizable.
%
\subsection{Example}\label{example:ex1} 
Consider the IVP
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated explicitly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta(x) = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x p_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1.
\end{equation}
%
where $p_\zeta$, associate with $r = \psi^2$, are given by 
%
\begin{equation*}
p_0 = \psi_0^2,~~~~~p_1 = 2\psi_0\psi_1,~~~~~p_2 = \psi_1^2 + 2\psi_0\psi_2
\end{equation*}
and so on. After a few evaluations, \eqref{eq:seriessol} leads to the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which one recognizes as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha} 
$$
Hence,
$$
\lim_{M\to \infty} \frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1\\
|x|,~&~\alpha = 1\\
\end{cases}
$$
Thus, convergence is linear. For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
The solution is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the the quality of PI approximations is better than ADM's. In essence, the rate of convergence of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is rather subtle. The following results provide some formal theoretical justifications of the method using the benchmark problem.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $p_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $U_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, it follows from  \eqref{eq:adommatchingun} that  
%
\begin{equation}\label{eq:stab}
\| \nabla \hat{\psi}_\zeta\|_{L^{2}(\Omega)} \leq  \delta_{\zeta0}C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + (1 - \delta_{\zeta0}) C_{\Omega,\zeta}\|p_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation}
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $U_\zeta$.
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\| \nabla (\psi - \hat{\psi}_M)\|_{L^2(\Omega)} \to 0$ as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Since $\psi$ solve \eqref{eq:vf} and $\hat{\psi}_M$ is a partial solution, it follows that 
%
$$
a(\hat\psi_M, w) + \sum_{\zeta < M} (p_\zeta, w) = \ell(w).
$$
Also, the truncation error $e_M = \psi - \hat{\psi}_M$ satisfies
%
$$
a(e_M,w) = b(\psi; w) - \sum_{\zeta < M} (p_\zeta, w) = \sum_{\zeta \geq M} (p_\zeta, w)
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, the following result holds:
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)} 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} 
$$
The theorem follows as $\sum_{\zeta \geq M} p_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that if the zeroth mode of the ADM and the beginning condition of PI coincide, then the two methods are identical as long as $r$ is linear. This results was first established by Golberg \cite{golberg1999note}. The major setback of his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $p_{\zeta} = r(\psi_{\zeta}) = \psi_{\zeta}$ for all $\zeta \geq 0$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. Then 
%
\begin{equation*}
\begin{split}
a(\hat{\psi}_M - \tilde{\psi}_M,w) &= a(\hat{\psi}_M,w) - a(\tilde{\psi}_M,w) \\
& = \Big(\ell(w) - \sum_{\zeta < M} (p_\zeta, w)\Big) -  \Big(\ell(w) - (r(\tilde{\psi}_{M-1}), w) \Big)\\
& = \Big(\ell(w) - \sum_{\zeta < M} (\psi_\zeta, w)\Big) -  \Big(\ell(w) -  (\tilde{\psi}_{M-1}, w) \Big)\\
& = (\tilde{\psi}_{M-1}, w) - (\hat{\psi}_{M-1}, w)\\
& = 0
\end{split}
\end{equation*}
%
As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to place restrictions on $p_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $u_D = 0$, it is known that there is at least one nontrivial solution. Here, $p_\zeta = 0$ for all $\zeta$, so the partial solution converges to the trivial solution. It is noteworthy that the trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely, for instance, by adding and and subtracting an artificial source term to unsure that the first mode is nonzero. 
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the algorithm above using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: This is a Sine-Gordon problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity is $r = -\sin u$ and $f$ is chosen such that the exact solution is 
$$
u = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6].
$$

\noindent
\textbf{Test 2}: A Helmholtz-type problem with boundary conditions $u = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~u = 0~\text{on}~\Gamma_{N}^R$ and $u = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$. Moreover, we set $r = u$ and $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$ so that the exact solution is 
$$
u = \cos(2\pi x) \sin(2\pi y).
$$

\noindent
\textbf{Test 3}: A Modified Ginzburg-Landau problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity $r = u - u^3$ is prescribed and $f$ is constructed accordingly such that the exact solution is $u = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Bratu problem with boundary conditions $ u = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $u = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$. We also set $r = -2\exp(u)$ and choose $f$ such that exact solution is 
$$
u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~\text{ where}~~\theta = 2\cosh(0.25 \theta)
$$

\subsection{Numerical approximations}
It is fascinating that numerical results produced by the ADM are almost identical to those obtained using Picard iteration. For this reason, an attempt is made to evaluate the performance (in terms of number of iterations and error) of the two methods. In particular, for a fixed element area, the ADM algorithm is run until the stopping criterion $\|\mathcal{R}(\sum_{m=0}^{M} U_m)\| \leq 10^{-10}$ is met. To match the the same operations with PI, we equate solving for one mode of the ADM approximation to one iteration of PI. The stopping criterion $\| \mathcal{R}(\boldsymbol  \alpha_{m})\|_\infty \leq 10^{-10}$ is used to for PI.\\[1ex]
%


\noindent
\textbf{Test 1}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
Except for $n = 8$ elements, the approximations from both methods are again consistent. Even though the ADM with $8$ elements has smaller error, the method fails to converge. In fact, $\|\mathcal{R}(\bfs{\alpha}_{m})\|_\infty$ plateaues out at $3.8462\times 10^{-3}$ and convergence is never attained. At this point, additional terms scarcely improve the partial solutions. This clearly results from the numerical treatment but not a limitation of the method.
%



\subsection{Numerical convergence study}\label{sec:conv}
%
We perform numerical convergence study of the ADM and PI.\\[1ex]
\noindent
\textbf{Test 1}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex1error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error1}
\end{figure}

%
\noindent
\textbf{Test 2}:\\
\subsubsection{Test 2:}
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex2error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error2}
\end{figure}

%
\noindent
\textbf{Test 3}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex3error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error3}
\end{figure}



%
\noindent
\textbf{Test 4}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex4error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error4}
\end{figure}
















\subsection{Discussions}\label{sec:discusion}

It is apparently that the exponential convergence of the Adomian decomposition suggested by some studies is not supported by these results. As iterated above, exponential convergence may be validated using simple one-dimensional Cauchy problems. For complicated nonlinearities however, the Adomian decomposition is no more appealing as the associated polynomials are are difficult to evaluate analytically. For BVPs, the exercises in this study confirms that convergence of the method is generally linear and almost consistent with Picard iteration, except when the first mode of the partial solution deviates significantly from the exact solution. Largely, the first mode inherits the most important features of the solution. As it departs from the exact solution substantially, not only do we observe a reduced convergence, accuracy is also affected adversely.  








%
Evidently, the approximations compare favorably with the exact solution. It is remarkable that the errors associated with the ADM and PI are commensurate  and consistently of the same order. However, the VADM (especially in 1D applications) sometimes show insignificant improvements over the PI. \\[1ex]



Unlike the former test, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Golberg's conclusion holds. The two schemes may differ in scope but their approximations do not vary significantly. \\[1ex] 
%



\section{Conclusion} \label{sec:conclusion}
The Adomian decomposition has been explored numerically from a variational context. While the method has been characterized as super convergent and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI. However, the test problems presented in this paper show that it is indeterminate to conclude that the ADM converges faster and provides superior approximations. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method completely avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems in lower and higher dimensions. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for other explorations. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Moreover, superior approximations and fast convergence of the ADM over its counterpart, the Picard Iteration, is not been supported by this study.\\[1ex] 






























































%We solve a modified stationary Ginzburg-Landau-type problem with homogeneous Dirichlet conditions. The nonlinear reaction is $r(x,u) = u - u^3$. As emphasized above, analytical solutions to this problem are unknown and non-unique. 
%Calculation of $\mathcal{P}_\zeta$ in this example is less tedious as it is easy to automatize the process. Simulation results are depicted in the following figure and table.

















\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}





%This procedure is summarized in the following table.
%%
%\begin{algorithm}[H]
%\caption{ADM procedure}
%\begin{algorithmic}
%\smallskip
%\State Find $u_0 = v - u_D \in H^1_\text{D}(\Omega)$ satisfying  $A(u_0,w) = L(w)$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\For{$\zeta = 1$} until convergence
%\smallskip
%\State Find $u_\zeta \in H^1_\text{D}(\Omega)$ satisfying  $A(u_\zeta,w) + J_{\zeta-1}(w) = 0$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\EndFor
%\smallskip
%\State Set $u = \sum_{\zeta=0}^\infty u_{\zeta}$.
%\end{algorithmic}\label{alg:adomianvf}
%\end{algorithm}














%\textbf{Example 1}
%Consider the Bratu problem 
%%
%\begin{equation}\label{eq:bratu}
%-u'' - 2\exp(u) = 0,~~u(0) = u(1) = 0.
%\end{equation}
%%
%with solution 
%\begin{equation*}
%u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~~~\text{where}~~~~\theta = 2\cosh(0.25 \theta)
%\end{equation*}
%%
%Clearly, the first mode of the ADM is trivial since it solves $-u_0'' = 0, ~u_0(0) = u_0(1) = 0$. Accordingly, the first few Adomian polynomials are 
%%
%\begin{equation}\label{eq:bratuadompolyn}
%\begin{split}
%p_0 & = 2\exp(u_0) = 2,\\
%p_1 & = 2 u_1 \exp(u_0) = 2 u_1,\\
%p_2 & = 2 u_2 \exp(u_0) + u_1^2 \exp(u_0) = 2 u_2 + u_1^2,\\ 
%\end{split}
%\end{equation}
%%
%and so on. One primary advantage of the ADM that comes handy is that we are able to calculate the modes exactly or semi-analytically. Here, the higher-order modes given explicitly by
%%
%\begin{equation}\label{eq:seriessol}
%u_\zeta = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
%\end{equation}
%%
%Table \ref{tab:adom1} shows the errors associated with the first five nontrivial partial solutions.
%%
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.88630(-02)& 7.38115(-03)& 3.13039(-03)& 1.39757(-03)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five partial solution.}}\label{tab:adom1}
%\end{center}
%%
%For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. Then,  the $M^{\text{th}}$-iterate is calculated according to
%%
%\begin{equation}\label{eq:pibratu}
%-\psi_M'' - 2\exp(\psi_{M-1}) = 0, ~~\text{with}~~~\psi_M(0) = \psi_M(1) = 0.
%\end{equation}
%%
%The solution follows \eqref{eq:seriessol} with $p_{\zeta-1}$ replaced by $\exp(\psi_{\zeta-1})$. However, except $\psi_0$, all higher-order iterates are available semi-analytically. The associated errors are also tabulate in Table \ref{tab:picard1}.
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\psi_M$  & $\psi_1$ & $\psi_2$ & $\psi_3$ & $\psi_4$ & $\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.45576(-02)& 3.89215(-03)& 1.04761(-03)& 2.82658(-04)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
%\end{center}
%%
%Apparently, the two schemes maintain the same order of accuracy. However, PI approximations show marginal gains over ADM's. This is because $u_0 \equiv 0$ leads to slow convergence of the associated polynomials (see \eqref{eq:bratuadompolyn}), which in turn results in loss in accuracy.



\section{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration (also known as simple or fixed-point iteration). Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. It has also been documented that the ADM converges exponentially. As mentioned earlier, majority of convergence studies used simple forms of $r$ which makes it possible to infer the exact solution from the first few partial solutions. This study does not attempt to unify the two methods. Rather, it provides the framework to appreciate the convergence rates of the two schemes. To provide a common ground and access the performance the schemes, we provide a simple tests to demonstrate that superiority of one of the methods is problem dependent and not generalizable.\\[1ex]
%
\textbf{Example 1}
Consider the modified stationary Gross-Pitaevskii problem
%
\begin{equation}
\begin{split}
-\psi'' - 2\psi^3 + \psi &= 0,~~x \in (0,1),\\[1ex]
\psi(0) = 1,~ \psi(1) &= 2e/(1+e^2)
\end{split}
\end{equation}
%
which is satisfied  by $\psi(x) = \sech x$. With $r = -2\psi^3 + \psi $, the associated Adomian polynomials are 
%
\begin{equation*}
\begin{split}
p_0 &= -2\psi_0^3 + \psi_0,\\
p_1 &= - 6\psi_1\psi_0^2 + \psi_1,\\
p_2 &= - 6\psi_2\psi_0^2 - 6\psi_0\psi_1^2 + \psi_2,
\end{split}
\end{equation*}
and so on. The zeroth mode solves 
$$
-\hat\psi_0'' = 0,~~~~\hat\psi_0(0) = 1,~ ~\hat\psi_0(1) = 2e/(1+e^2)
$$ 
with solution 
$$
\hat\psi_0(x) = (1 + (1 - x)e^2 - x + 2ex))/(1 + e^2)
$$
All higher order terms are calculated using
%
\begin{equation}\label{eq:gensol}
\hat\psi_\zeta(x) = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
\end{equation}
%
Table \ref{tab:adom1} shows the errors associated with the first five partial solutions.
%
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $6.51945(-03)$ & $2.86278(-03)$  & $1.33711(-03)$ \\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five partial solution calculated using $N = 64$ elements.}}\label{tab:adom1}
\end{center}
%
For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. The $M^{\text{th}}$-iterate satisfies
%
\begin{equation}\label{eq:pibratu}
-\tilde \psi_M'' - 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1} = 0, ~~\text{with}~~~\tilde \psi_M(0) = 1,~~\tilde \psi_M(1) = 2e/(1+e^2).
\end{equation}
%
The solution follows \eqref{eq:gensol} with $p_{\zeta-1}$ replaced by $- 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1}$. The associated errors are also tabulate in Table \ref{tab:picard1}.
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\tilde\psi_M$  & $\tilde\psi_1$ & $\tilde\psi_2$ & $\tilde\psi_3$ & $\tilde\psi_4$ & $\tilde\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $5.96274(-03)$ & $2.22830(-03)$ & $8.43414(-04)$\\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
\end{center}




==> manuscriptold.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE On the comparison of the Adomian decomposition and Picard Iteration
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}

There has been a long held controversy about the equivalence of the Adomian Decomposition Method and Picard Iteration. Even though  studies suggest that convergence of the Adomian Decomposition Method is faster than Picard Iteration and the quality of approximations is superior, recent investigations suggest otherwise. This work examines the performance of the two methods with semilinear boundary value problems which are important kernels in many numerical applications. Theoretical justifications are provided and supported by several numerical experiments. The test problems presented demonstrate that even though the two methods are distinctive, they produce approximations of nearly the same quality. However, the exponential convergence of the Adomian Decomposition Method suggested by some studies is not supported.
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the comparison between the Adomian decomposition (ADM) and Picard Iteration (PI) using the benchmark problem
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) = f,~~~~~&x\in \Omega,\\
\psi = \psi_D,~~~~~&x\in \Gamma_D,\\
-n\cdot \nabla \psi = g_N,~~~~~&x\in \Gamma_N.
\end{split}
\end{equation}
Here, $\Omega$ is a bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundary conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. 
%
\par In a variety of context, \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. They include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in some coordinate systems, which allow solutions to be written in closed form. However, the fundamental models governing most natural phenomena involving motion, diffusion, reaction, etc. occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of a numerical scheme with some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for the model problem \eqref{eq:bvp} do not always produce satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 
%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated. In many studies, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumptions on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito explored the existence of entire solutions by enforcing separability of $r$ and the unknown. He assumed that $r$ is expressible as $r = a(x)g(w)$, where $a$ is locally H\"older on $\R^n$ and $f$ (which is positive and nondecreasing for $w>0$) is a locally Lipschitz and continuous function on $\R^+$. In the said article, he established approximate range of the limit values of positive solutions. In later studies, his results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was also studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Infinitely many solutions may also exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory on nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible when major components of the mathematical model are trivialized, realistic models are relatively complicated and rarely admit closed form solutions. In spite of this, advances in differential and integro-differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods relies on the conjecture that solutions to nonlinear equations can be expressed as series. This leads to a set of explicit recursive relations governing the modes of the series. Methods of this sort are robust for approximating solutions to IVPs, but have been reformulated to adapt to boundary and initial boundary-value problems. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solutions. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par The Adomian Decomposition Method (ADM) has dominated the discussion about analytical methods recently. A lot of problems have been explored with the ADM and results were impressive. Interestingly, it is argued that in some tests the ADM yields the exact solution within few steps. This is debatable since those studies use simple functional forms of $r$.  This simplification makes it possible to write the series solution in closed form. What has not been discussed adequately is the fact that for complicated problems, the mode of the series may not be solvable analytically. Even if closed form expressions exist for the modes, it may not be possible to write the limit of the partial sum in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat misleading. One of the objectives of this study is to provide theoretical results on the convergence of the ADM from a variational perspective. This study also attempts to compare the ADM with Picard Iteration which shares a lot of conceptual and practical similarities. The remainder of the paper is organized as follows: Section \ref{sec:vf} discusses the weak and Galerkin approximation of \eqref{eq:bvp}. An iterative method is developed in Section \ref{eq:im} and compared with Picard Iteration. Theoretical results are also provided and supported by several test problems in Section \ref{sec:experiments}. Section \ref{sec:discusion} concludes the study with a brief overview of the performance of the ADM and Picard iteration.
%
\section{Weak formulation}\label{sec:wf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $\psi_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads:
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla u \cdot \nabla w \,\d x + \int_\Omega r(\cdot, u)w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x,~~ w \in H^1_\text{D}(\Omega).
\end{split}
\end{equation}
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,\psi) = r(\psi)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\subsection{Galerkin approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is:
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&\int_\Omega \nabla u_h \cdot \nabla w_h \,\d x + \int_\Omega r(\cdot, u_h)w_h \,\d x = \int_\Omega fw_h \d x + \int_{\Gamma_N} gw_h\, \d l - \int_\Omega \nabla \psi_{D,h} \cdot \nabla w_h\, \d x,~~w_h \in \mathcal{V}_{\text{D},h}^k.
\end{split}
\end{equation}
%
Here, $\psi_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is the nodal approximation of $\psi_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N,~|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
\psi_{D,h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. $\mathcal{A}$ is a square matrix and $\mathcal{B}(\bfs{\alpha})$, a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x~~~\text{and}~~~\mathcal{B}_\zeta(\bfs{\alpha}) = \int_\Omega r(\sum \alpha_z \phi_z) \phi_\zeta \,\d x.
\end{equation}
%
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ are also given by 
%
\begin{equation}
\beta_\zeta = \int_\Omega f\phi_{\zeta}\, dx,~~~~\gamma_\zeta = \int_{\Gamma_N} g \phi_{\zeta}\, dl,~~~~\mathcal{D}_{\zeta z} = \int_\Omega \nabla \phi_z \cdot \nabla \phi_\zeta\, \d x,~~~z \in Z,~\zeta \in \tilde{Z}.
\end{equation}
%
The Galerkin solution that approximates $\psi$ is written as
%
\begin{equation}
U = u_h + \psi_{D,h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix makes Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}\label{eq:im}
We furnish the weak form in \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem into a sequential inversion of the Laplacian. To begin, suppose that $\psi$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode $\psi_0$. Explicitly,
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} \mathcal{P}_\zeta
\end{equation}
%
where $\psi_\zeta,~\zeta \geq 0$ are to be determined. The terms $\mathcal{P}_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
\mathcal{P}_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $\mathcal{P}_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
 \sum_{\zeta \geq 0} \left(\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x + \int_\Omega \mathcal{P}_\zeta w \,\d x \right) = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x.
\end{equation}
%
The iterative scheme is developed by constructing the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ via matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem:
%
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&~\text{Find $\psi_\zeta = \varphi - \delta_{\zeta0}\psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \psi_\zeta \cdot \nabla w \,\d x +  (1 - \delta_{\zeta0})\int_\Omega \mathcal{P}_\zeta w \,\d x = \delta_{\zeta0}\left(\int_\Omega fw \,\d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x\right)
\end{split}
\end{equation}
%
where $\varphi$ solve \eqref{eq:bvp} with $r = 0$, $\mathcal{P}_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, $\psi_0$ absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $\mathcal{P}_\zeta$ depends on $\psi_j,~ 0\leq j \leq \zeta-1$ only, $\mathcal{P}_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \sum_{\zeta \leq M} \psi_\zeta.
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved is summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  + \boldsymbol{F}_{\zeta-1} = 0$,~~where $\boldsymbol{F}_{\zeta z} = \int_\Omega \mathcal{P}_{\zeta} \phi_z \, \d x$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
Certainly, the ADM is attractive in the following ways: First, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. From \eqref{eq:adompolyn}, one observes that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grow exponentially. Also, a lot of memory is required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\subsection{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves the approximation of nonlinear equations by a sequence of explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the ADM and PI, where the majority of comparisons concluded that the ADM is the better of the two methods. Existing literature also suggest that the ADM is superconvergent (since it yields exact solutions within few iterations) and involves less computational work. This mischaracterization motivates some discussions in this study. First, analytical solutions are possible only when one is able to identify the partial solution with a familiar Taylor series. If the terms are mixed up and do not follow a recognizable series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:vf} generates the sequence $\{\tilde\psi_\zeta\}$ governed by the variational problem: 
%
\begin{equation}\label{eq:vfpicard}
\begin{split}
&~\text{Find $\tilde\psi_M = \varphi - \psi_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&\int_\Omega \nabla \tilde\psi_M \cdot \nabla w \,\d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x - \int_\Omega r(\tilde\psi_{M-1})w \,\d x,
\end{split}
\end{equation}
%
for a specified beginning condition $\tilde\psi_{-1}$. The resulting Galerkin discrete problem is summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple test demonstrates that superiority of the ADM (as documented in some literature) is not supported and cannot be generalized.
%
\subsection{Example}\label{example:ex1} 
Consider the problem
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated exactly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x \mathcal{P}_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1,
\end{equation}
%
where $\mathcal{P}_\zeta$, associated with $r = \psi^2$, are given by 
%
\begin{equation*}
\mathcal{P}_0 = \psi_0^2,~~~~~\mathcal{P}_1 = 2\psi_0\psi_1,~~~~~\mathcal{P}_2 = \psi_1^2 + 2\psi_0\psi_2,~~\cdots.
\end{equation*}
After few evaluations, we obtain the the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which is recognized as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the exact solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha}. 
$$
It follows that 
$$
\lim_{M\to \infty} \frac{|\hat\psi_{M+1} - \psi|}{|\hat\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1,\\
|x|,~&~\alpha = 1.\\
\end{cases}
$$
Thus, convergence is linear for the ADM. 
\par For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
If the beginning condition $\tilde\psi_{-1} = 0$ is supplied so that $\tilde\psi_0$ is consistent with ADM's zeroth mode, then $\tilde\psi_M$ is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta > M}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the quality of PI approximations is better than ADM's. Overall, the convergence rate of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is subtle. The following results provide theoretical justifications that, for sufficient regularity conditions, the modes of the ADM are controlled and the partial solution converges to the exact solution.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $\psi_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, then 
$$
\| \nabla {\psi}_0\|_{L^{2}(\Omega)} \leq  C_{\Omega,0}\|f\|_{L^{2}(\Omega)} 
$$
and 
$$
\| \nabla {\psi}_\zeta\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta =1,2,\cdots,M
$$
%
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $\psi_\zeta$. It follows that  
%
\begin{equation*}
\| \nabla \hat{\psi}_M\|_{L^{2}(\Omega)} \leq  C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + \sum_{\zeta \leq M} C_{\Omega,\zeta}\|\mathcal{P}_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation*}
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\hat{\psi}_M \to \psi$ in $H^1$ norm as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $\mathcal{P}_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Now, since $\psi$ satisfy \eqref{eq:vf} and $\hat\psi_M$ satisfies
%
\begin{equation*}
\int_{\Omega} \nabla \hat\psi_M \cdot \nabla w\, \d x + \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \int_\Omega fw \d x + \int_{\Gamma_N} gw\, \d l - \int_\Omega \nabla \psi_D \cdot \nabla w\, \d x 
\end{equation*}
the error $e_M = \psi - \hat{\psi}_M$ satisfies
$$
\int_{\Omega} \nabla e_M \cdot \nabla w\, \d x = \int_\Omega r(\psi)w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x = \sum_{\zeta \geq M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x.
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, it holds that 
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|\mathcal{P}_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)}. 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|\mathcal{P}_\zeta\|_{L^2(\Omega)}. 
$$
The theorem follows as $\sum_{\zeta \geq M} \mathcal{P}_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that whenever the zeroth mode of the ADM and the beginning condition of PI coincide, the two methods are identical as long as $r$ is linear. This result was first established by Golberg \cite{golberg1999note}. The major setback to his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}\label{lemm:lemmaadpisame}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $\mathcal{P}_\zeta = r(\psi_\zeta) = \psi_\zeta$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. After cancelling out common terms, we have 
%
\begin{equation*}
\begin{split}
\int_{\Omega} \nabla(\hat{\psi}_M - \tilde{\psi}_M) \cdot \nabla w\, \d x & = \int_{\Omega} \nabla \hat{\psi}_M\cdot \nabla w\, \d x - \int_{\Omega} \nabla \tilde{\psi}_M\cdot \nabla w\, \d x,\\
&=  \int_\Omega r(\tilde\psi_{M-1})w \,\d x - \sum_{\zeta < M} \int_{\Omega} \mathcal{P}_\zeta w \, \d x,\\
& =  \int_\Omega \tilde\psi_{M-1} w\,\d x - \int_\Omega \hat\psi_{M-1} w\,\d x.
\end{split}
\end{equation*}
%
The last equation is zero by assumption. As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to impose additional restrictions on $\mathcal{P}_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $\psi_D = 0$, it is known that there is at least one nontrivial solution. A quick exercise shows that $\mathcal{P}_\zeta = 0$ for all $\zeta$, and hence, the partial solution converges to the trivial solution. A trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely.
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the ADM and PI algorithms using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: Boundary conditions: $\psi_D = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; ~Nonlinearity: $r = -\sin \psi$; ~$f$: chosen appropriately;~Solution: $\psi = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6]$.\\[1ex]

\noindent
\textbf{Test 2}: Boundary conditions: $\psi = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~\psi = 0~\text{on}~\Gamma_{N}^R$ and $\psi = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$;~ Nonlinearity:  $r = -\psi$;~ $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$;~ Solution:~ $\psi = \cos(2\pi x) \sin(2\pi y)$.\\[1ex]

\noindent
\textbf{Test 3}: Boundary conditions: $\psi = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$; Nonlinearity: $r = \psi - \psi^3$; ~$f$: chosen appropriately;~Solution $\psi = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Boundary conditions: $\psi = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $\psi = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$;~Nonlinearity: $r = -2\exp(\psi)$;~$f$: chosen appropriately;~Solution: $\psi = -2\ln[\cosh(0.25(2x-1)\theta)]/\cosh(0.25 \theta)$ where $\theta = 2\cosh(0.25 \theta)$.

\subsection{Numerical approximations}
For a fixed element area, the ADM and PI algorithms are run until the stopping criteria $\|\mathcal{R}(\hat\psi_M)\| \leq 10^{-10}$ and $\|\mathcal{R}(\tilde\psi_M)\| \leq 10^{-10}$ are met respectively.\\[1ex]
%


\newpage
\noindent
\textbf{Test 1}:\\
\vspace*{-0.15in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%

\newpage
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
\vspace*{0.5in}
%

\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small ADM and PI approximations compared with the analytical solution.}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Number of iterations recorded for the ADM and PI for various number of elements.}}
\end{center}
%

\newpage
\subsection{Numerical convergence study}\label{sec:conv}
%
\vspace*{-0.3in}
We perform numerical convergence study of the ADM and PI.\\[1ex]
%
\noindent
\textbf{Test 1}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex1error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error1}
\end{centering}
\end{figure}
\vspace*{-0.1in}



%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex2error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error2}
\end{centering}
\end{figure}
\vspace*{-0.2in}

%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex3error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error3}
\end{centering}
\end{figure}
\vspace*{0.3in}


%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.25in}
\begin{figure}[h!]
\begin{centering}
\centerline{\includegraphics[height=2.4in, width=2.8in]{figs/ex4error}}
\vspace*{-0.1in}
 \caption {\small Element area versus $L^2$-error of the ADM and PI approximations.}
  \label{fig:error4}
\end{centering}
\end{figure}

\subsection{Discussions and conclusion}\label{sec:discusion}
%
The numerical experiments show that the ADM approximations compare favorably with the analytical solutions. It is fascinating that the quality of the approximations obtained using the ADM and PI are commensurate. However, exponential convergence of the ADM suggested by some studies is not supported. For complicated nonlinearities however, the ADM is no more appealing as the associated polynomials are laborious to evaluate. In Test 3, the method fails to converge for $N = 8$ elements. The error $\|\mathcal{R}(\tilde\psi_M)\|_\infty$ plateaus out at $3.8462\times 10^{-3}$ and convergence is never attained, and additional terms scarcely improve the partial solution. It is noteworthy that this anomaly results from the numerical treatment but not a limitation of the method. 

\par The most important feature of the ADM revealed by this study is that convergence is generally linear and consistent with Picard iteration. In Test 2, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Lemma \ref{lemm:lemmaadpisame} and Golberg's conclusion holds. Indeed, the two schemes differ in scope but the quality of their approximations does not vary significantly. Contrary to the first three tests, Test 4 is intended to explore when PI can outperform the ADM. First of all, $\psi_0$ is the trivial solution. This leads to slow convergence of the associated Adomian polynomials. That is 
%
\begin{equation}\label{eq:bratuadompolyn}
\begin{split}
\mathcal{P}_0 & = 2\exp(\psi_0) = 2,\\
\mathcal{P}_1 & = 2 u_1 \exp(\psi_0) = 2 \psi_1,\\
\mathcal{P}_2 & = 2 u_2 \exp(\psi_0) + \psi_1^2 \exp(\psi_0) = 2 \psi_2 + \psi_1^2,\\ 
\mathcal{P}_3 & = \frac{1}{3}\psi_1^3 \exp(\psi_0) + 2\psi_3\exp(\psi_0) + 2\psi_1 \psi_2 \exp(\psi_0) = \frac{1}{3}\psi_1^3 + 2\psi_3 + 2\psi_1 \psi_2,
\end{split}
\end{equation}
and so on. Largely, the first mode of the partial solution inherits the most important features of the solution. As $\psi_0$ deviates significantly, convergence is affected adversely. One way to avoid this is to introduce, say, $f_1$ and $f_2$ into the differential equation such that $f_1 + f_2 = 0$. This way, the governing equation for $\psi_0$ may be written to have either $f_1$ as source term. $f_2$ is then expressed as a Taylor series and the terms are matched with the Adomian polynomials.\\[1ex]
%
\par The ADM and PI have been explored numerically from a variational context. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for exploring other nonlinear systems. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Even though the ADM is characterized as superconvergent, and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI.






\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}

==> update.tex <==
\input{packs}
\DeclareMathOperator{\sech}{sech}
\begin{document}
\begin{center}
{\LARGE A variational iterative scheme for semilinear boundary value problems
}\\[2em]

{Prosper Torsu\\ \em{Department of Mathematics, California State University, Bakersfield, CA 93311, USA}}
 
\end{center}

\begin{abstract}
This paper presents an iterative method for solving semilinear boundary-value problems, which are important kernels in many numerical applications. The method employs a decomposition that is able to reduce the original problem into a set of simpler problems which are easy to invert. For special boundary condition, the approach allows fast Poisson solvers to be engaged. Theoretical justifications are provided and supported by several numerical experiments. Results obtained suggest that the method is not only computationally attractive, but also produces accurate approximations.  
\end{abstract}

\noindent \textit{Keywords}: Semilinear two-point BVP, Finite element method, Adomian polynomials, Picard Iteration


\section{Introduction}
The object of discussion in this article is the boundary-value problem (BVP)
%
\begin{equation} \label{eq:bvp}
\begin{split}
-\Delta \psi + r(x, \psi) &= f,~~~~~\,x\in \Omega,\\
\psi &= \psi_\alpha,~~~x\in \Gamma_D,\\
-n\cdot \nabla \psi &= g_N,~~~x\in \Gamma_N,
\end{split}
\end{equation}
where $\Omega$ is bounded region with boundary $\partial \Omega$ and, $\Gamma_D$ and $\Gamma_D$ are respectively disjoint segments of $\partial \Omega$ identified with Dirichlet and Neumann boundaries conditions. Also, $n$ is the unit outward normal vector on $\Gamma_N$, $f$ and $g$ are known continuous data and $r:\Omega \times \R \to \R$ is continuously differentiable. In a variety of context, the model in \eqref{eq:bvp} is of great importance to mathematicians, physicists, biologists, engineers and other practitioners for modeling natural and human-induced phenomena. Models arising in this form describe steady-state characterization of evolution processes and have been the subject of extensive research in recent years. Some of the most commonly encountered classical mathematical models are classified as \eqref{eq:bvp}. These include the well-known Helmholtz equation, Bratu, Poisson-Boltzmann, the stationary Klein-Gordon, Allen-Cahn equation and Schr\"{o}dinger equations. Precisely, applications arise in, but not limited to the study of electrostatic properties \cite{baker2001electrostatics} and the study of acoustic and electromagnetic scattering \cite{colton2012inverse, martin2006multiple, voon2004helmholtz}. In the sphere of fluid dynamics, many models (e.g. the Implicit Pressure, Explicit Saturation formulation of water-oil displacement \cite{hasle2007geometric}) are governed by variants of \eqref{eq:bvp}.
%
\par Indeed, simpler variations of \eqref{eq:bvp} are separable in most coordinate systems, which allows solutions to be written in closed form. However, the fundamental models governing most natural phenomena (involving combinations of motion, diffusion, reaction, etc) occur nonlinearly. Despite their pivotal contribution to the evolution of mathematical theories and experimentation, analytical methods have served minimal roles as only a handful of realistic models have known solutions. For several decades now, scientific computation has  provided critical information about a wide class of problems that would otherwise be unavailable via analytical means. From a computational standpoint, solving \eqref{eq:bvp} requires the simultaneous application of some numerical scheme alongside some sort of iterative procedure to an associated discrete algebraic system. As it is known, classical central and upwind schemes for model problems of the form \eqref{eq:bvp} do not give satisfactory approximations. This is due to the inherent complex dynamics of $r$ leading to numerical challenges such as the appearance of singular effects \cite{amrein2015fully, roos2008robust}. Even though these numerical tools are very successful, resolving instabilities for stable and accurate approximations often require a lot of computational time and large amounts of memory. 

%
\par Far from a computational perspective is the issue of existence, solvability, uniqueness, regularity and number of solutions to \eqref{eq:bvp}. Nonlinear differential equations, in general, do not yield easily to rigorous and consolidated mathematical analysis because nonlinearities can be very complicated and chaotic. In many applications, solutions do not exist globally. Successful investigations into existence and uniqueness of solutions have also relied on rigid assumption on $r$ and $f$. For instance, in the article \cite{naito1984note}, Naito investigated the existence of entire solutions by enforcing separability of $r$ in the spatial coordinates and the unknown. In particular, the form $r = a(x)g(w)$ was assumed, where $a$ is locally H\"older on $\R^n$ and $f$ is a locally Lipschitz continuous function on $\R^+$ which is positive and nondecreasing for $w>0$. In the said article, the author established approximate range of the limit values of positive solutions. Naito's results were improved by Usami \cite{usami1986bounded}, where the general form $r = g(x,w,\nabla w)$ was considered. A more general case was studied by Boccardo and co. \cite{boccardo2010semilinear}. Their study proved the existence and regularity of \eqref{eq:bvp} with a non-constant conductivity and $r = f(x)w^{-\gamma}$, where $\gamma >0$. The article concluded that a locally and strictly positive distributional solution to \eqref{eq:bvp} exists if $f \in L^1(\Omega)$. A related familiar  discussion that runs across the aforementioned studies (also see \cite{amrein2015fully, badiale2010semilinear, lions1982existence}) is the existence of multiple nontrivial solutions even under very restrictive assumptions. Sometimes, infinitely many solutions exist \cite{kusano1986entire,ni1982elliptic}. Even though extensive study of special classes of nonlinear differential equations exist today, there is no unified theory of nonlinear equations \cite{rosinger2015can}. 
%
\par Naturally, analytical solutions to differential equations are desired. While this is possible only when major components of the mathematical model are trivialized, realistic models are relatively complicated do not generally permit closed form solutions. In spite of this, advances in differential equations saw the light of novel analytical techniques \cite{adomian1990review, aryana2018series, MR1934316, MR2199322, wazwaz1998comparison, yildirim2010he}. The heart of these methods is to conjecture that solutions to nonlinear equations can be expressed as infinite series. This leads to a set of explicit recursive relations governing the modes of the series. These methods are robust for approximating solutions to Cauchy problems but has been reformulated to adapt to boundary and initial boundary-value problems. In some test problems, these methods have been demonstrated to yield the exact solutions. Certainly, the principal theme that has dominated most discussions about these techniques is the rapid convergence of the series solution. Despite this conception, important questions about convergence of the method are still open because related studies are mainly problem-specific and do not provide a unifying ground to generalize convergence results. 
%
\par It is debatable that the methods yield exact solutions in some problems because simple functional forms are used.  This simplification makes it possible to write the series solutions in closed forms. What has not been discussed adequately is the fact that for complicated problems, the systems governing each mode of the partial solution may not be solvable analytically. Moreover, even if closed form expressions exist for the modes, it may not be possible to write the limit of the approximation in a compact form because the partial solution may not follow a known Taylor series. In such occurrences, the notion of fast convergence is delicate and somewhat subtle. One of the objectives of this study is to provide a variational framework for studying the convergence of the Adomian Decomposition Method (ADM) which shares a lot of similarities with other decomposition techniques. Once the framework is established, all finite element results follow readily. This study will also attempt to compare the ADM to Picard Iteration (PI). While the two methods are distinct in their conceptual and practical approaches, the later has been considered by some authors as superior. This study will compare the performance of the two methods numerically. The remainder of the paper is organized as follows: Section \ref{sec:motivation} provides a simple motivation which inspires this discussion. Section \ref{sec:vf} discusses the Galerkin approximation that is used to invert \eqref{eq:bvp}. The numerical procedures that use the Adomian decomposition and Picard Iteration are outlined in Section \ref{sec:discralg}. Section \ref{sec:experiments} explores several numerical experiments to compare the performance of the two methods; and Section \ref{sec:conclusion} concludes the study with a brief overview.
%















\section{Weak formulation}\label{sec:vf}
%
We consider a bounded Lipschitz domain $\Omega \subset \R^2$ with polygonal boundary  $\partial \Omega$ which is decomposed as $\partial \Omega = \Gamma_D \cup \Gamma_N$, with $|\Gamma_D|>0$. Suppose that $u_D \in H^1(\Omega), g_N \in L^2(\Gamma_N)$ and define 
%
\begin{equation*}
H^1_\text{D}(\Omega) = \big\{ w \in H^1(\Omega) : w|_{\Gamma_D}  = 0\big\}.
\end{equation*}
%
Given $f \in L^2(\Omega)$, and under the assumption that a solution (not necessarily unique) exists, the weak formulation associated with \eqref{eq:bvp} reads
%
\begin{equation}\label{eq:vf}
\begin{split}
&~\text{Find $u = \psi - u_\text{D} \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&~a(u,w) + b(u; w)= \ell(w),~~~ \forall w \in H^1_\text{D}(\Omega),
\end{split}
\end{equation}
%
where
%
\begin{equation}\label{eq:vdef}
\begin{split}
&a(v,w) = (\nabla v, \nabla w),\\[1ex]
&b(v;w) = (r(\cdot,v), w),\\[1ex]
&\ell(w) = (f,w) - \langle g,w\rangle_N - a(u_D,w).
\end{split}
\end{equation}
%
Here, $(\cdot,\cdot)$ denotes the usual inner product in $L^2(\Omega)$ and $\langle \cdot, \cdot \rangle_N$ is
the inner product on $L^2(\Gamma_N)$. 
%
In the sequel, the explicit dependence of $r$ on $x$ is ignored and we write $r(x,u) = r(u)$ for brevity. An important step towards the construction of the finite element solution consists of approximating the continuous problem in \eqref{eq:vf} by seeking the solution on a finite dimensional subspace of $H^1_\text{D}(\Omega)$. Mainly, $H^1_\text{D}(\Omega)$ is replaced by the set of piecewise continuous polynomials with compact support. 
%
\section{Galerkin finite element approximation}\label{sec:vf}
Consider a triangulation $\Tau_h$ of $\Omega$ such that  ${\overline \Omega}=\cup_{\tau \in {\Tau}_h} \tau$ with $h=\max_{\tau \in {\Tau}_h} \{h_\tau\}$ and $h_\tau=\sqrt{|\tau|}$. The finite element space associated with ${\Tau}_h$ is defined as
%
\begin{equation}
\mathcal{V}^k_h= \{w_h\in C({\overline {\Omega }}): w_h|_\tau \in \mathcal{V}_k(\tau)
\text{ for all } \tau \in {\Tau}_h\} \subset H^1(\Omega),
\end{equation}
%
where $\mathcal{V}_k(\tau)$ is an appropriate space of polynomials with degree less than or equal to $k$. Denote $\mathcal{V}_{\text{D},h}^k = \mathcal{V}_h^k \cap H^1_\text{D}(\Omega)$. Then, that the finite element approximation is
%
\begin{equation} \label{eq:fem}
\begin{split}
&~\text{Find $u_h \in \mathcal{V}_{\text{D},h}^k$ satisfying}\\[1ex]
&~a(u_h, w_h) + b(u_h; w_h) = \ell(w_h),~~~ \forall w_h \in \mathcal{V}_{\text{D},h}^k,
\end{split}
\end{equation}
%
where $a$ and $b$ satisfy \eqref{eq:vdef} and 
\begin{equation}
\ell(w_h) = (f,w_h) - \langle g, w_h \rangle_N - a(u_{D,h},w_h)
\end{equation}
%
Here, $u_{\text{D},h} \in \mathcal{V}_{\text{D},h}^k$ is used as an approximation (e.g. nodal interpolant) of $u_D$ on $\Gamma_D$. Let $Z$ be the set of degrees of freedom
associated with $\mathcal{V}_h^k$ and $\tilde{Z}$ be the set of degrees of freedom associated with $\widetilde{\V}$
such that $\tilde{Z} \subset Z$, respectively having $|Z| = N$ and $|\tilde{Z}| = \tilde{N}$ and $\tilde{N} < N$. We then identity that 

%
\begin{equation}
\mathcal{V}_h^k = \text{span} \big\{ \phi_z \big\}_{z \in Z} ~~~~~~\text{and} ~~~~~~
\mathcal{V}_{\text{D},h}^k = \text{span} \big\{ \phi_z \big\}_{z \in \tilde{Z}},
\end{equation}
%
where $\phi_z$ is the finite element basis function that is associated with the degree of freedom $z$. By setting
%
\begin{equation}
u_h = \sum_{z \in \tilde{Z}} \alpha_z \phi_z ~~~~~~ \text{and} ~~~~~~
u_{\text{D},h} = \sum_{z \in Z} \alpha_{\text{D},z} \phi_z,
\end{equation}
%
the variational problem in \eqref{eq:fem} reduces to the discrete algebraic equation 
%
\begin{equation}\label{eq:nonlinsys}
\mathcal{R}(\bfs{\alpha}) = \mathcal{A}\bfs{\alpha} + \mathcal{B}(\bfs{\alpha}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = 0
\end{equation}
%
which governs $\bfs{\alpha} \in \mathbb{R}^{\tilde{N}}$. The matrix $\mathcal{A}$ is square and $\mathcal{B}(\bfs{\alpha})$ is a matrix function whose entries are respectively given by 
%
\begin{equation}
\mathcal{A}_{\zeta z} =  a(\phi_z, \phi_\zeta)~~~\text{and}~~~ \mathcal{B}_\zeta(\bfs{\alpha}) = b(\sum \alpha_z \phi_z; \phi_\zeta)
\end{equation}
The vectors $\bfs{\beta}, \bfs{\gamma} \in \mathbb{R}^{\tilde{N}}$ and the matrix $\mathcal{D}\in M_{\tilde{N} \times N}(\R)$ also have entries 
%
\begin{equation}
\beta_\zeta = (f, \phi_{\zeta}),~~~~~\gamma_\zeta = \<g_N, \phi_{\zeta}\>_N,~~~~\mathcal{D}_{\zeta z} = a(\phi_z, \phi_\zeta),~~z \in Z,~\zeta \in \tilde{Z}
\end{equation}
%
The Galerkin finite element solution that approximates $\widetilde{u}$ is written as
%
\begin{equation}
\tilde{u}_h = u_h + u_{\text{D},h} =  \sum_{z \in \tilde{Z}} \alpha_z \phi_z + \sum_{z \in Z} \alpha_{\text{D},z} \phi_z.
\end{equation}
%
As $\mathcal{R}$ is nonlinear, direct inversion of \eqref{eq:nonlinsys} requires the use of some iterative procedure. Standard practice involves the application of some quadrature rules alongside a linearization scheme. With appropriate regularity conditions, Newton methods guarantee higher convergence and are generally preferred. However, the laborious and unavoidable calculation of the associated jacobian matrix make Newton methods the unappealing when results are needed in a short timeframe. Beside Picard iterations which converge slower but easier to implement, analytical methods have also been utilized to easily obtain qualitative features of solutions to nonlinear problems.  Discussed in the next section is a decomposition which provides an alternative iterative machinery for inverting \eqref{eq:nonlinsys} without actually linearizing $\mathcal{R}$. 

\section{An iterative approach}
We furnish the weak form \eqref{eq:vf} with the ADM other than the conventional application to the differential equation. This makes it possible to reduce the nonlinear problem in \eqref{eq:vf} into a sequential inversion of the Laplacian. To begin, let $u$ satisfy \eqref{eq:bvp} and $v$ solve a similar problem with $r = 0$. Suppose in addition that $u$ is expressible as an infinite series and $r$ is written as a generalized Taylor series around the zeroth mode. That is
%
\begin{equation}\label{eq:uapolyseries} 
\psi  =  \sum_{\zeta \geq 0} \psi_\zeta~~~~\text{and}~~~~r =  \sum_{\zeta \geq 0} p_\zeta
\end{equation}
%
where $\psi_0$ (referred to as the zeroth) and $\psi_\zeta,~\zeta \geq 1$ are to be determined. The terms $p_\zeta$ are the Adomian polynomials associated with $r$, and are determined explicitly using the formula
%
\begin{equation}\label{eq:adompolyn}
p_\zeta = \frac{1}{\zeta!} \frac{\textrm{d}^{\zeta}}{\textrm{d} \lambda^{\zeta}} \Big[r\Big(\sum_{j \geq 0} \lambda^j 
\psi_j \Big) \Big]_{\lambda = 0}.
\end{equation}
%
It is evident that $p_\zeta$ depends on $\psi_j,~0 \leq j \leq \zeta - 1$. Upon substituting \eqref{eq:uapolyseries} into \eqref{eq:vf}, the variational equation can be written in the form 
%
\begin{equation}\label{eq:adomdecompo}
a(\psi_0,w) + \sum _{\zeta \geq 1}\big[a(\psi_\zeta,w) + (p_{\zeta}, w)\big] = \ell(w).
\end{equation}
%
The iterative scheme is developed by finding the sequence $\{\psi_\zeta\}_{\zeta = 0}^\infty$ by matching terms in \eqref{eq:adomdecompo} such that $\psi_\zeta$ solves the variational problem
%
\begin{equation}\label{eq:adommatchingun} 
\begin{split}
&\text{Find $\psi_\zeta = v - \delta_{\zeta0}u_D \in H^1_\text{D}(\Omega)$ satisfying}\\[1ex]
&a(\psi_\zeta,w) + (1 - \delta_{\zeta0}) (p_{\zeta-1}, w) = \delta_{\zeta0}\ell(w),~~~\zeta = 0,1,2, \cdots.
\end{split}
\end{equation}
%
where $p_{-1} = 0$ and $\delta$ is the Kronecker delta. Here, the zeroth mode absorbs the boundary conditions of the original problem. All higher order terms serve as corrections to the approximation $\psi = \psi_0$ and honor the same boundary structure but homogeneous conditions. As $p_\zeta$ depends on $\psi_j,~ \leq j \leq \zeta-1$ only, $p_{\zeta-1}$ in the equation for $\psi_\zeta$ is known. As a result, inversion of $r$ amounts to a sequence of inversions of the Laplacian. The practical solution is given by the $M$-term partial solution
%
\begin{equation}
\hat\psi_M = \psi_0 + \sum_{\zeta \geq 1} \psi_\zeta
\end{equation}
%
Upon a successful Galerkin discretization, the discrete problem to be solved can be summarized as follows:
%
\begin{algorithm}[H]
\caption{ADM approximation}
\begin{algorithmic}
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_0 = \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D}$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A}\bfs{\Psi}_\zeta  = \bfs{\xi}_{\zeta-1}$,~~where ${\xi}_{\zeta z} = - (p_{\zeta}, \phi_z)$.
\smallskip
\EndFor
\smallskip
\State Set $\hat{\bfs{\Psi}}_M = \bfs{\Psi}_0 + \sum_{\zeta \leq M} \bfs{\Psi}_{\zeta}$.
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
Certainly, the ADM is attractive in the following ways: First of all, the inversion of the nonlinear problem \eqref{eq:nonlinsys} is replaced by a repeated inversion of the Laplacian. This can be done efficiently especially when the boundary conditions are special, e.g., pure Dirichlet or pure Neumann. This way, discrete sine or cosine transforms can be engaged to accelerate calculation of the modes. Secondly, since the decomposition is performed on the variational equation, the approach is applicable to other boundary types with equal success. In addition, any potential difficulty associated with the imposition of boundary conditions using the classical ADM is avoided entirely. However, it is observed that the method is no longer attractive for complicated functional forms of $r$ as the cost of calculating the associated polynomials can grows exponentially. A lot of memory is also required as all lower order solutions are required to calculate higher order ones. Notwithstanding, fast algorithms for calculating the polynomials exist today.

\section{Comparison with Picard Iteration}
Perhaps the most familiar iteration is the Picard Iteration. Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. 
\par Another aspect of the ADM that has been mischaracterized is its convergence. The method has been portrayed as superconvergent by many authors even though this assessment is misleading for an arbitrary nonlinearity. In fact, a closed form solution is possible only when one is able to identify the function whose truncated Taylor series is represented by the partial solution. If the terms are mixed up and do not follow a recognizable Taylor series, one is forced to obtain a partial sum other than the exact solution. It is important in this respect to know what kind of convergence to expect. This study shows that convergence of the ADM is generally linear and the quality of the approximations is comparable to PI approximations. 
%
\par In this context, the PI approximation of \eqref{eq:nonlinsys} generates the sequence $\{\tilde\psi_\zeta\}$ governed by 
%
\begin{equation}\label{eq:picarditer} 
\begin{split}
&\text{Find $\tilde\psi_M = v - \psi_D \in H^1_\text{D}(\Omega)$ satisfying }\\[1ex]
&a(\tilde\psi_\zeta,w) =  \ell(w) - (r(\tilde\psi_{\zeta-1}), w),~~~\forall w\in H^1_\text{D}(\Omega)
\end{split}
\end{equation}
%
for a specified beginning condition $u_0$. The resulting discrete problem can be summarized as follows:
%
\begin{algorithm}[H]
\caption{Picard Iteration}
\begin{algorithmic}
\smallskip
\State Set $\tilde{\bfs{\Psi}}_0$.
\smallskip
\For{$\zeta = 1$} until convergence
\smallskip
\State Solve $\mathcal{A} \tilde{\bfs{\Psi}}_\zeta + \mathcal{B}(\tilde{\bfs{\Psi}}_{\zeta-1}) + \bfs{\beta} + \bfs{\gamma} + \mathcal{D}\bfs{\alpha}_\text{D} = \0$.
\smallskip
\EndFor
\smallskip
\end{algorithmic}\label{alg:adomianvf}
\end{algorithm}
%
\noindent 
To provide a common ground and access the performance the two schemes, the following simple tests demonstrates that superiority of one of the methods is not definite generalizable.
%
\subsection{Example}\label{example:ex1} 
Consider the IVP
\begin{equation*}
\psi' - \psi^2 = 0,~~~~\psi(0) = 1
\end{equation*}
%
with exact solution $\psi(x) = 1/(1 - x)$. With the classical ADM, the modes of the partial solution are calculated explicitly using the formula
%
\begin{equation}\label{eq:seriessol}
\psi_\zeta(x) = \delta_{0\zeta} + (1 - \delta_{0\zeta}) \int_0^x p_{\zeta-1}\, \d \xi,~~~~\zeta \geq 1.
\end{equation}
%
where $p_\zeta$, associate with $r = \psi^2$, are given by 
%
\begin{equation*}
p_0 = \psi_0^2,~~~~~p_1 = 2\psi_0\psi_1,~~~~~p_2 = \psi_1^2 + 2\psi_0\psi_2
\end{equation*}
and so on. After a few evaluations, \eqref{eq:seriessol} leads to the partial solution
\begin{equation*}
\hat\psi_M = \sum_{\zeta\leq M} x^\zeta
\end{equation*}
%
which one recognizes as the partial sum of the exact solution. Thus, we are able to write down an explicit formula for the solution after a few terms because $\hat\psi_M$ is a familiar partial sum. However, this does not constitute fast convergence. We note that for a fixed $x$,
$$
\frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = \frac{|x^{M+2}/(1-x)|}{|x^{M+1}/(1-x)|^\alpha} = 
|x-1|^{\alpha -1} |x|^{2 + M - (1 + M) \alpha} 
$$
Hence,
$$
\lim_{M\to \infty} \frac{|\psi_{M+1} - \psi|}{|\psi_{M} - \psi|^\alpha} = 
\begin{cases}
\infty,~&~\alpha > 1\\
|x|,~&~\alpha = 1\\
\end{cases}
$$
Thus, convergence is linear. For Picard Iteration on the other hand, the $M^{\text{th}}$ iterate is given by the formula
%
\begin{equation}\label{eq:picarddemo}
\tilde\psi_M(x) = 1 + \int_0^x \tilde\psi^2_{M-1} \, \d \xi,~~~~M \geq 1.
\end{equation} 
%
The solution is expressible in the form 
$$
\tilde\psi_M(x) = \sum_{\zeta\leq M} x^\zeta + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta = \hat\psi_{M}(x) + \sum_{\zeta = M+1}^{2^{M}-1} a_\zeta x^\zeta
$$ 
where $1 \gtrapprox a_{M+1} > a_{M+2} > \cdots > a_{2^M-1}  \gtrapprox 0$. Since the number of terms doubles and one additional term is corrected after each iteration, the the quality of PI approximations is better than ADM's. In essence, the rate of convergence of the ADM correlates strongly with convergence of the associated Adomian polynomials. Since there is no multipurpose class of Adomian polynomials, the notion of fast convergence is rather subtle. The following results provide some formal theoretical justifications of the method using the benchmark problem.
%
\begin{lemma} \label{lem:stability}
Let $\hat{\psi}_M$ be the partial solution obtained using the ADM. Then, $\hat{\psi}_M$ is stable provided $p_\zeta \in L^2(\Omega)$ for all ~$0 \leq \zeta \leq M$. 
\end{lemma}
%
\begin{proof}
Stability is immediate from Poincar\'e inequality. For, if $U_\zeta, ~0 \leq \zeta \leq M$, are the modes of $\hat{\psi}_M$, it follows from  \eqref{eq:adommatchingun} that  
%
\begin{equation}\label{eq:stab}
\| \nabla \hat{\psi}_\zeta\|_{L^{2}(\Omega)} \leq  \delta_{\zeta0}C_{\Omega,\zeta}\|f\|_{L^{2}(\Omega)} + (1 - \delta_{\zeta0}) C_{\Omega,\zeta}\|p_{\zeta-1}\|_{L^{2}(\Omega)},~~~\zeta = 0,1,2,\cdots
\end{equation}
where $C_{\Omega,\zeta},~\zeta = 0,1,2\cdots$ are independent of $U_\zeta$.
\end{proof}
%

\begin{lemma} \label{lem:lem2}
Let $\psi$ satisfy \eqref{eq:vf} and $\hat{\psi}_M$ be a partial solution obtained using the ADM. Then $\hat{\psi}_M$ is unique provided $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$. Moreover, $\| \nabla (\psi - \hat{\psi}_M)\|_{L^2(\Omega)} \to 0$ as $M \to \infty$.
%
\end{lemma}
%
\begin{proof}
As $p_\zeta \in L^2(\Omega)$ for all $0 \leq \zeta \leq M$, Lax-Milgram guarantees the existence and uniqueness of $\psi_\zeta,~0 \leq \zeta \leq M$ and hence the uniqueness of $\hat{\psi}_M$. Since $\psi$ solve \eqref{eq:vf} and $\hat{\psi}_M$ is a partial solution, it follows that 
%
$$
a(\hat\psi_M, w) + \sum_{\zeta < M} (p_\zeta, w) = \ell(w).
$$
Also, the truncation error $e_M = \psi - \hat{\psi}_M$ satisfies
%
$$
a(e_M,w) = b(\psi; w) - \sum_{\zeta < M} (p_\zeta, w) = \sum_{\zeta \geq M} (p_\zeta, w)
$$
%
By virtue of Cauchy-Schwarz, triangle and Poincar\'e inequalities, the following result holds:
%
\begin{equation*}
\begin{split}
\|\nabla e_M\|^2_{L^2(\Omega)} &\leq \Bigg(\sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|e_M\|_{L^2(\Omega)} \leq \Bigg(\sum_{\zeta \geq M} \|p_\zeta\|_{L^2(\Omega)} \Bigg) \|\nabla e_M\|_{L^2(\Omega)} 
\end{split}
\end{equation*}
%
Consequently, 
$$
\|\nabla e_M\|_{L^2(\Omega)} \leq \sum_{\zeta \geq M}  \|p_\zeta\|_{L^2(\Omega)} 
$$
The theorem follows as $\sum_{\zeta \geq M} p_\zeta \to 0$ for sufficiently large $M$.
\end{proof}
%
\noindent 
The following result shows that if the zeroth mode of the ADM and the beginning condition of PI coincide, then the two methods are identical as long as $r$ is linear. This results was first established by Golberg \cite{golberg1999note}. The major setback of his findings is that his  results pertain to linear forms of $r$, and does not extend to arbitrary nonlinearity in general.
%
\begin{lemma}
Let $\hat{\psi}_M$ and $\tilde{\psi}_M$ be the approximations obtained using the ADM and PI respectively. If $r$ is linear and $\hat{\psi}_0 = \tilde{\psi}_0$, then $\tilde{\psi}_M = \hat{\psi}_M$ holds for all $M\geq 1$. 
\end{lemma}
\begin{proof}
By linearity of $r$, we must have $p_{\zeta} = r(\psi_{\zeta}) = \psi_{\zeta}$ for all $\zeta \geq 0$. Suppose, for the sake of induction, that $ \hat{\psi}_{M-1} = \tilde{\psi}_{M-1}$ for $M \geq 2$. Then 
%
\begin{equation*}
\begin{split}
a(\hat{\psi}_M - \tilde{\psi}_M,w) &= a(\hat{\psi}_M,w) - a(\tilde{\psi}_M,w) \\
& = \Big(\ell(w) - \sum_{\zeta < M} (p_\zeta, w)\Big) -  \Big(\ell(w) - (r(\tilde{\psi}_{M-1}), w) \Big)\\
& = \Big(\ell(w) - \sum_{\zeta < M} (\psi_\zeta, w)\Big) -  \Big(\ell(w) -  (\tilde{\psi}_{M-1}, w) \Big)\\
& = (\tilde{\psi}_{M-1}, w) - (\hat{\psi}_{M-1}, w)\\
& = 0
\end{split}
\end{equation*}
%
As this holds for arbitrary $w\in H^1_\text{D}(\Omega)$, it must be that $\tilde{\psi}_M - \hat{\psi}_M$ is constant in $H^1_\text{D}(\Omega)$. We then deduce that $\tilde{\psi}_M - \hat{\psi}_M = 0$. This completes the proof.
\end{proof}
\noindent 
%
\begin{remark}\textnormal{
It is apparent from Example \ref{example:ex1} that the manner in which the two schemes update the iterates differ. While PI has the capability to investigate the existence of a solution, the traditional ADM does not always yield nontrivial approximations. There are several problems where it is necessary to place restrictions on $p_\zeta$ to guarantee a nonzero solution. For instance, by setting $r = \psi^3 - \psi$ and $u_D = 0$, it is known that there is at least one nontrivial solution. Here, $p_\zeta = 0$ for all $\zeta$, so the partial solution converges to the trivial solution. It is noteworthy that the trivial solution can be avoided by simply altering the beginning condition for PI. However, the ADM must be modified completely, for instance, by adding and and subtracting an artificial source term to unsure that the first mode is nonzero. 
}
\end{remark}
%
\section{Numerical study}\label{sec:experiments}
We test the algorithm above using the following test problems. Even though the problems are manufactured and may not bear any physical meaning, they do  provide good insights into the performance of the method.\\[1ex]
%
\textbf{Test 1}: This is a Sine-Gordon problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity is $r = -\sin u$ and $f$ is chosen such that the exact solution is 
$$
u = 10(x-x^2)(y-y^2)\tan^{-1}[100(x-y)^6].
$$

\noindent
\textbf{Test 2}: A Helmholtz-type problem with boundary conditions $u = \sin 2\pi y~\text{on}~~\Gamma_{D}^L,~u = 0~\text{on}~\Gamma_{N}^R$ and $u = 0~\text{on}~\Gamma_{D}^B \cup \Gamma_{D}^T$. Moreover, we set $r = u$ and $f = (8\pi^2 - 1) \cos(2\pi x) \sin(2\pi y)$ so that the exact solution is 
$$
u = \cos(2\pi x) \sin(2\pi y).
$$

\noindent
\textbf{Test 3}: A Modified Ginzburg-Landau problem with boundary conditions $u = 0~\text{on}~~\Gamma_{D}^L \cup \Gamma_{D}^B \cup \Gamma_{D}^R \cup \Gamma_{D}^T$. The nonlinearity $r = u - u^3$ is prescribed and $f$ is constructed accordingly such that the exact solution is $u = \omega(x)\omega(y)$, where 
$$
\omega(s) = 1 + \exp(-1/0.05) - \exp(-s/0.05) - \exp((s - 1)/0.05). 
$$

\noindent
\textbf{Test 4}: Bratu problem with boundary conditions $ u = 0~\text{on}~\Gamma_{D}^L \cup \Gamma_{D}^R$ and $u = 0 ~\text{on}~\Gamma_{N}^B \cup \Gamma_{N}^T$. We also set $r = -2\exp(u)$ and choose $f$ such that exact solution is 
$$
u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~\text{ where}~~\theta = 2\cosh(0.25 \theta)
$$

\subsection{Numerical approximations}
It is fascinating that numerical results produced by the ADM are almost identical to those obtained using Picard iteration. For this reason, an attempt is made to evaluate the performance (in terms of number of iterations and error) of the two methods. In particular, for a fixed element area, the ADM algorithm is run until the stopping criterion $\|\mathcal{R}(\sum_{m=0}^{M} U_m)\| \leq 10^{-10}$ is met. To match the the same operations with PI, we equate solving for one mode of the ADM approximation to one iteration of PI. The stopping criterion $\| \mathcal{R}(\boldsymbol  \alpha_{m})\|_\infty \leq 10^{-10}$ is used to for PI.\\[1ex]
%


\noindent
\textbf{Test 1}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex1exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx1}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $8$ & $8$ & $7$ & $7$ & $6$\\[1ex] 
 PICARD  & $8$ & $8$ & $7$ & $7$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular} 
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 2}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex2exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx2}
\end{figure}
%
\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 VADM       & $9$ & $8$ & $7$ & $6$ & $6$\\[1ex] 
 PICARD  & $9$ & $8$ & $7$ & $6$ & $6$ \\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 3}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex3exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx3}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $\infty$ & $12$ & $9$ & $8$ & $7$ \\[1ex] 
 PICARD  & $24$ & $12$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
\noindent
\textbf{Test 4}:\\
\vspace*{-0.1in}
%
\begin{figure}[h!]
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4ad}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4pi}}\hspace*{2in}
\makebox[0pt][l]{\includegraphics[height=1.7in, width=2in]{figs/ex4exact}}
\vspace*{-0.02in}
 \caption {\small VADM approximation (Left) compared with the exact solution (Right).}
 \label{fig:approx4}
\end{figure}

\begin{center}
\begin{tabular}{cccccc}
\toprule
  & $8~\text{elements}$ & $16~\text{elements}$ & $32~\text{elements}$ & $64~\text{elements}$ & $128~\text{elements}$ \\ 
 \hline\\[-1.5ex]
 ADM       & $18$ & $17$ & $15$ & $13$ & $11$ \\[1ex] 
 PICARD  & $11$ & $10$ & $9$ & $8$ & $7$\\[0.5ex]
\bottomrule
\end{tabular}
\captionof{table}{\small{Performance of ADM and PI compared in terms of number of iterations and $L^2$-error.}}
\end{center}
%
Except for $n = 8$ elements, the approximations from both methods are again consistent. Even though the ADM with $8$ elements has smaller error, the method fails to converge. In fact, $\|\mathcal{R}(\bfs{\alpha}_{m})\|_\infty$ plateaues out at $3.8462\times 10^{-3}$ and convergence is never attained. At this point, additional terms scarcely improve the partial solutions. This clearly results from the numerical treatment but not a limitation of the method.
%



\subsection{Numerical convergence study}\label{sec:conv}
%
We perform numerical convergence study of the ADM and PI.\\[1ex]
\noindent
\textbf{Test 1}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex1error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error1}
\end{figure}

%
\noindent
\textbf{Test 2}:\\
\subsubsection{Test 2:}
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex2error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error2}
\end{figure}

%
\noindent
\textbf{Test 3}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex3error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error3}
\end{figure}



%
\noindent
\textbf{Test 4}:\\
\begin{figure}[h!]
\hspace*{1.5in}
\makebox[0pt][l]{\includegraphics[height=2.6in, width=3.2in]{figs/ex4error}}
\vspace*{-0.02in}
 \caption {\small Element area versus $L^2$-error of some approximation obtained using the VADM.}
 \label{fig:error4}
\end{figure}
















\subsection{Discussions}\label{sec:discusion}

It is apparently that the exponential convergence of the Adomian decomposition suggested by some studies is not supported by these results. As iterated above, exponential convergence may be validated using simple one-dimensional Cauchy problems. For complicated nonlinearities however, the Adomian decomposition is no more appealing as the associated polynomials are are difficult to evaluate analytically. For BVPs, the exercises in this study confirms that convergence of the method is generally linear and almost consistent with Picard iteration, except when the first mode of the partial solution deviates significantly from the exact solution. Largely, the first mode inherits the most important features of the solution. As it departs from the exact solution substantially, not only do we observe a reduced convergence, accuracy is also affected adversely.  








%
Evidently, the approximations compare favorably with the exact solution. It is remarkable that the errors associated with the ADM and PI are commensurate  and consistently of the same order. However, the VADM (especially in 1D applications) sometimes show insignificant improvements over the PI. \\[1ex]



Unlike the former test, identical performance of the two methods is unsurprising. This should be anticipated because $r$ is linear, in which case, Golberg's conclusion holds. The two schemes may differ in scope but their approximations do not vary significantly. \\[1ex] 
%



\section{Conclusion} \label{sec:conclusion}
The Adomian decomposition has been explored numerically from a variational context. While the method has been characterized as super convergent and the better of the two methods, numerical experiments demonstrate that the method is more or less as accurate as the Picard iteration. The ADM, in practice, offers more flexibility over PI. However, the test problems presented in this paper show that it is indeterminate to conclude that the ADM converges faster and provides superior approximations. In strong form, inversion of a nonlinear differential operator is replaced by a series of inversions of the discrete Laplacian. This is appealing because the method completely avoids the nontrivial task of calculating the associated Jacobian matrix. Although the formulation is confined to the benchmark problems, it is extensible to other types of problems in lower and higher dimensions. Results obtained provide an alternative way of analyzing the ADM and provide firm grounds for other explorations. As confirmed by the numerical experiments, the ADM formulation functions flawlessly and adapts easily to various boundary types. Moreover, superior approximations and fast convergence of the ADM over its counterpart, the Picard Iteration, is not been supported by this study.\\[1ex] 






























































%We solve a modified stationary Ginzburg-Landau-type problem with homogeneous Dirichlet conditions. The nonlinear reaction is $r(x,u) = u - u^3$. As emphasized above, analytical solutions to this problem are unknown and non-unique. 
%Calculation of $\mathcal{P}_\zeta$ in this example is less tedious as it is easy to automatize the process. Simulation results are depicted in the following figure and table.

















\bibliographystyle{siam}
\bibliography{biblio} 
\end{document}





%This procedure is summarized in the following table.
%%
%\begin{algorithm}[H]
%\caption{ADM procedure}
%\begin{algorithmic}
%\smallskip
%\State Find $u_0 = v - u_D \in H^1_\text{D}(\Omega)$ satisfying  $A(u_0,w) = L(w)$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\For{$\zeta = 1$} until convergence
%\smallskip
%\State Find $u_\zeta \in H^1_\text{D}(\Omega)$ satisfying  $A(u_\zeta,w) + J_{\zeta-1}(w) = 0$, for all $w\in H^1_\text{D}(\Omega)$.
%\smallskip
%\EndFor
%\smallskip
%\State Set $u = \sum_{\zeta=0}^\infty u_{\zeta}$.
%\end{algorithmic}\label{alg:adomianvf}
%\end{algorithm}














%\textbf{Example 1}
%Consider the Bratu problem 
%%
%\begin{equation}\label{eq:bratu}
%-u'' - 2\exp(u) = 0,~~u(0) = u(1) = 0.
%\end{equation}
%%
%with solution 
%\begin{equation*}
%u = -\frac{2\ln[\cosh(0.25(2x-1)\theta)]}{\cosh(0.25 \theta)},~~~~\text{where}~~~~\theta = 2\cosh(0.25 \theta)
%\end{equation*}
%%
%Clearly, the first mode of the ADM is trivial since it solves $-u_0'' = 0, ~u_0(0) = u_0(1) = 0$. Accordingly, the first few Adomian polynomials are 
%%
%\begin{equation}\label{eq:bratuadompolyn}
%\begin{split}
%p_0 & = 2\exp(u_0) = 2,\\
%p_1 & = 2 u_1 \exp(u_0) = 2 u_1,\\
%p_2 & = 2 u_2 \exp(u_0) + u_1^2 \exp(u_0) = 2 u_2 + u_1^2,\\ 
%\end{split}
%\end{equation}
%%
%and so on. One primary advantage of the ADM that comes handy is that we are able to calculate the modes exactly or semi-analytically. Here, the higher-order modes given explicitly by
%%
%\begin{equation}\label{eq:seriessol}
%u_\zeta = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
%\end{equation}
%%
%Table \ref{tab:adom1} shows the errors associated with the first five nontrivial partial solutions.
%%
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.88630(-02)& 7.38115(-03)& 3.13039(-03)& 1.39757(-03)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five partial solution.}}\label{tab:adom1}
%\end{center}
%%
%For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. Then,  the $M^{\text{th}}$-iterate is calculated according to
%%
%\begin{equation}\label{eq:pibratu}
%-\psi_M'' - 2\exp(\psi_{M-1}) = 0, ~~\text{with}~~~\psi_M(0) = \psi_M(1) = 0.
%\end{equation}
%%
%The solution follows \eqref{eq:seriessol} with $p_{\zeta-1}$ replaced by $\exp(\psi_{\zeta-1})$. However, except $\psi_0$, all higher-order iterates are available semi-analytically. The associated errors are also tabulate in Table \ref{tab:picard1}.
%\begin{center}
%\begin{tabular}{lccccc}
%\toprule
%$\psi_M$  & $\psi_1$ & $\psi_2$ & $\psi_3$ & $\psi_4$ & $\psi_5$ \\ 
% \hline\\[-1.5ex]
%Error   & 5.58326(-02)& 1.45576(-02)& 3.89215(-03)& 1.04761(-03)& 2.82658(-04)\\[1ex] 
%\bottomrule
%\end{tabular}
%\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
%\end{center}
%%
%Apparently, the two schemes maintain the same order of accuracy. However, PI approximations show marginal gains over ADM's. This is because $u_0 \equiv 0$ leads to slow convergence of the associated polynomials (see \eqref{eq:bratuadompolyn}), which in turn results in loss in accuracy.



\section{Comparison with Picard Iteration (PI)}
Perhaps the most familiar iteration is the Picard Iteration (also known as simple or fixed-point iteration). Analogous to ADM, PI involves approximation of nonlinear equations via successive explicit evaluations subject to some beginning condition. There has been a long held controversy about the equivalence of the two approaches and the ADM has been adjudged by many authors as the better. Existing literature \cite{elsaid2012fractional, evans2002new, kaya1999solution} suggests that the ADM involves less computational work and yields exact solutions within few iterations. It has also been documented that the ADM converges exponentially. As mentioned earlier, majority of convergence studies used simple forms of $r$ which makes it possible to infer the exact solution from the first few partial solutions. This study does not attempt to unify the two methods. Rather, it provides the framework to appreciate the convergence rates of the two schemes. To provide a common ground and access the performance the schemes, we provide a simple tests to demonstrate that superiority of one of the methods is problem dependent and not generalizable.\\[1ex]
%
\textbf{Example 1}
Consider the modified stationary Gross-Pitaevskii problem
%
\begin{equation}
\begin{split}
-\psi'' - 2\psi^3 + \psi &= 0,~~x \in (0,1),\\[1ex]
\psi(0) = 1,~ \psi(1) &= 2e/(1+e^2)
\end{split}
\end{equation}
%
which is satisfied  by $\psi(x) = \sech x$. With $r = -2\psi^3 + \psi $, the associated Adomian polynomials are 
%
\begin{equation*}
\begin{split}
p_0 &= -2\psi_0^3 + \psi_0,\\
p_1 &= - 6\psi_1\psi_0^2 + \psi_1,\\
p_2 &= - 6\psi_2\psi_0^2 - 6\psi_0\psi_1^2 + \psi_2,
\end{split}
\end{equation*}
and so on. The zeroth mode solves 
$$
-\hat\psi_0'' = 0,~~~~\hat\psi_0(0) = 1,~ ~\hat\psi_0(1) = 2e/(1+e^2)
$$ 
with solution 
$$
\hat\psi_0(x) = (1 + (1 - x)e^2 - x + 2ex))/(1 + e^2)
$$
All higher order terms are calculated using
%
\begin{equation}\label{eq:gensol}
\hat\psi_\zeta(x) = \left(x\int_0^1 - \int_0^x \right)\left( \int_0^\xi p_{\zeta-1}(\tau) \d \tau \right) \d \xi ,~~~~\zeta \geq 1.
\end{equation}
%
Table \ref{tab:adom1} shows the errors associated with the first five partial solutions.
%
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\hat\psi_M$  & $\hat\psi_1$ & $\hat\psi_2$ & $\hat\psi_3$ & $\hat\psi_4$ & $\hat\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $6.51945(-03)$ & $2.86278(-03)$  & $1.33711(-03)$ \\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five partial solution calculated using $N = 64$ elements.}}\label{tab:adom1}
\end{center}
%
For the PI approximations, we prescribe the starting condition $\psi_0 \equiv 0$ consistent with the first mode of the ADM. The $M^{\text{th}}$-iterate satisfies
%
\begin{equation}\label{eq:pibratu}
-\tilde \psi_M'' - 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1} = 0, ~~\text{with}~~~\tilde \psi_M(0) = 1,~~\tilde \psi_M(1) = 2e/(1+e^2).
\end{equation}
%
The solution follows \eqref{eq:gensol} with $p_{\zeta-1}$ replaced by $- 2\tilde \psi_{M-1}^3 + \tilde \psi_{M-1}$. The associated errors are also tabulate in Table \ref{tab:picard1}.
\begin{center}
\begin{tabular}{lccccc}
\toprule
$\tilde\psi_M$  & $\tilde\psi_1$ & $\tilde\psi_2$ & $\tilde\psi_3$ & $\tilde\psi_4$ & $\tilde\psi_5$ \\ 
 \hline\\[-1.5ex]
$L^2$-Error   & $4.64166(-02)$ & $1.62462(-02)$ & $5.96274(-03)$ & $2.22830(-03)$ & $8.43414(-04)$\\[1ex] 
\bottomrule
\end{tabular}
\captionof{table}{\small{$L^2$-error of the first five iterates.}}\label{tab:picard1}
\end{center}



